Data-Driven Synthesis of Provably Sound Side Channel Analyses

We propose a data-driven method for synthesizing a static analyzer to detect side-channel information leaks in cryptographic software. Compared to the conventional way of manually crafting such a static analyzer, which can be labor intensive, error prone and suboptimal, our learning-based technique is not only automated but also provably sound. Our analyzer consists of a set of type-inference rules learned from the training data, i.e., example code snippets annotated with ground truth. Internally, we use syntax-guided synthesis (SyGuS) to generate new features and decision tree learning (DTL) to generate type-inference rules based on these features. We guarantee soundness by formally proving each learned rule via a technique called Datalog query containment checking. We have implemented our technique in the LLVM compiler and used it to detect power side channels in C programs. Our results show that, in addition to being automated and provably sound during synthesis, the learned analyzer also has the same empirical accuracy as two state-of-the-art, manually crafted analyzers while being 300X and 900X faster, respectively.

==> abstract.tex <==
\begin{abstract}
We propose a \emph{data-driven} method for synthesizing static
analyses to detect side-channel information leaks in cryptographic
software.  Compared to the conventional way of manually crafting such
static analyzers, which can be tedious, error prone and suboptimal,
our \emph{learning-based} technique is not only automated but also
provably sound.
%
Our analyzer consists of a set of type-inference rules learned from
the training data, i.e., example code snippets annotated with the ground
truth.  Internally, we use \emph{syntax-guided synthesis (SyGuS)} to
generate new recursive features and \emph{decision tree learning (DTL)} to
generate analysis rules based on these features.  We guarantee
soundness by proving each learned analysis rule via a technique called
\emph{query containment checking}.
%
We have implemented our technique in the LLVM compiler and used it to
detect \emph{power side channels} in C programs that implement
cryptographic protocols.  Our results show that, in addition to being
automated and provably sound during synthesis, our analyzer
can achieve the same empirical accuracy as two state-of-the-art,
manually-crafted analyzers while being 300X and 900X faster,
respectively.
\end{abstract}


==> conclusion.tex <==
%\vspace{-.5em}
\vspace{-.2em}
\section{Conclusions}
\label{sec:conclusion}
\vspace{-.2em}
We have presented a data-driven method for learning a \emph{provably
  sound} static analyzer, to detect power side channels in
cryptographic software.  It relies on SyGuS to generate new features
and DTL to generate type-inference rules based on the synthesized features.  It
verifies the soundness of the learned analysis rules by solving a Datalog query
containment checking problem using an SMT solver.
%
We have implemented and evaluated our method on C programs that implement
well-known cryptographic protocols and algorithms.
%
The experimental results show that our learning algorithm is efficient
and our learned analyzer can achieve the same empirical accuracy as
state-of-the-art, hand-crafted analysis tools while 
%being several hundred times faster.
being several orders-of-magnitudes faster.


==> experiments.tex <==
\section{Experiments}
\label{sec:experiment}

Our experiments were designed to answer the following research
questions (RQs):
\begin{itemize}
\item RQ1: How effective is our learned analyzer in terms of the analysis speed and accuracy?
\item RQ2: How effective is our method for learning  inference rules from training data?
\item RQ3: How effective is our method for proving the learned inference rules?
\end{itemize}

We implemented \GPS{} in LLVM 3.6.  \GPS{} relies on LLVM to parse the
C programs and construct the internal representation (IR).  Then, it
learns a static analyzer in two steps.  The first step, which is
SyGuS-guided decision tree learning, is implemented in 4,603 lines of
C++ code.  The second step, which proves the learned inference rules,
is implemented using the Z3~\cite{de2008z3} SMT solver.  Furthermore,
the learned analyzer (for detecting power side channels in
cryptographic software) is implemented in LLVM as an optimization
($opt$) pass.
%
We ran all experiments on a computer with 2.9 GHz Intel Core i5 CPU
and 8 GB RAM.  Our artifacts, including \GPS{} and all benchmarks,
will be published with the paper.


\subsection{Benchmarks} \label{subsec:benchmark}

Our benchmarks are 568 programs with 2,691K lines of C code in total.
They implement well-known cryptographic algorithms such as AES and SHA-3.
Some of these programs are hardened by countermeasures, such as
reordered MAC-Keccak computation ~\cite{bertoni2012keccak}, masked
AES~\cite{blomer2004provably,barthe2015verified}, masked S-box
calculation~\cite{coron2013higher} and masked
multiplication~\cite{rivain2010provably}, to eliminate side-channel
information leaks.


We partition the benchmarks into two sets: $D_{train}$ for \GPS{}, and
$D_{test}$ for the learned analyzer.
%
The training set $D_{train}$ consists of 531 small programs gathered
from various public sources, including byte-masked
AES~\cite{yao2018fault}, random reduction of
S-box~\cite{zhang2017further}, common shares~\cite{coron2016faster},
and leak examples~\cite{eldib2014synthesis}.  
Each benchmark is a pair consisting of program AST and its distribution type, i.e, the ground truth annotated by developers.
%The distribution type of
%each AST node is annotated by developers.
%
The testing set $D_{test}$ consists of 37 large programs, whose
statistics (the number of lines of code and inputs labeled public,
private, and random) are shown in Table~\ref{tbl:stats}.  Since these
programs are large, it is no longer practical to manually annotate the
ground truth; instead, we relies on the results of published tools: a
(manually-crafted) static analyzer~\cite{wang2019mitigating} for
B1-B20 and a formal verification tool~\cite{zhang2018sc} for B21-B37.
%While both tools are sound, they are significantly more expensive
%(100X to 1000X slower) than our learned analyzer.






\begin{comment}
\begin{table}
\caption{Statistics of the benchmark programs in $D_{test}$.}
\label{tbl:stats}
\centering
\scalebox{0.7}{
\begin{tabular}{|l|l|r|c|c|c|}
\hline
\multirow{2}{*}{Name} & \multirow{2}{*}{Description} & \multirow{2}{*}{LoC} & \multicolumn{3}{c|}{Input Variables}
\\ \cline{4-6}
 &    &           & $\mathit{I}_{pub}$ & $\mathit{I}_{priv}$ & $\mathit{I}_{rand}$
\\\hline\hline

B1  & AES Shift Rows          & 11    &0    &2          &2                     \\ \hline
B2  & Messerges Boolean       & 12    &0    &2          &2                     \\ \hline
B3  & Goubin Boolean          & 12    &0    &1          &2                     \\ \hline
B4  & SecMultOpt\_wires\_1    & 25    &1    &1          &3                     \\ \hline
B5  & SecMult\_wires\_1       & 25    &1    &1          &3                     \\ \hline
B6  & SecMultLinear\_wires\_1 & 32    &1    &1          &3                     \\ \hline
B7  & CPRR13-lut\_wires\_1    & 81    &1    &1          &7                     \\ \hline
B8  & CPRR13-OptLUT\_wires\_1 & 84    &1    &1          &7                     \\ \hline
B9  & CPRR13-1\_wires\_1      & 104   &1    &1          &7                     \\ \hline
B10 & KS\_transitions\_1      & 964   &1    &16         &32                    \\ \hline
B11 & KS\_wires           & 1,130     &1    &16         &32                    \\ \hline
B12 & keccakf\_1turn      & 1,256     &0    &25         &75                    \\ \hline
B13 & keccakf\_2turn      & 2,506     &0    &25         &125                   \\ \hline
B14 & keccakf\_3turn      & 3,764     &0    &25         &175                   \\ \hline
B15 & keccakf\_7turn      & 8,810     &0    &25         &349                   \\ \hline
B16 & keccakf\_11turn     & 13,810    &0    &25         &575                   \\ \hline
B17 & keccakf\_15turn     & 18,858    &0    &25         &775                   \\ \hline
B18 & keccakf\_19turn     & 23,912    &0    &25         &975                   \\ \hline
B19 & keccakf\_24turn     & 30,228    &0    &25         &1,225                 \\ \hline
B20 & AES\_wires\_1       & 34,358    &16    &16        &1,232                 \\  \hline \hline

B21 &Masked Key Whitening                &79   &0   &16  &16     \\ \hline
B22 &De-mask and then Mask               &67   &0   &8   &16     \\\hline
B23 &AES Shift Rows                      &21   &0   & 2  & 2     \\ \hline
B24 &Messerges Boolean to Arithmetic     &23   & 0  & 2  & 2     \\ \hline
B25 &Goubin Boolean to Arithmetic        &27   & 0  & 1  & 2     \\ \hline
B26 & Logic Design for AES S-Box(1)      &32   &0   & 2  & 2     \\ \hline
B27 & Logic Design for AES S-Box(2)      &40   &0   &2   & 3     \\ \hline
B28 & Masked Chi function MAC-Keccak (1) &59   & 0  & 3  & 4     \\ \hline
B29 & Syn. Masked Chi func MAC-Keccak(1) &66   &0   & 3  & 4     \\ \hline
B30 & Syn. Masked Chi func MAC-Keccak(2) &66   &0   & 3  & 4     \\ \hline
B31 & MAC-Keccak 512b De-mask \& mask    &426k &288 &288 &3,205  \\ \hline
\end{tabular}
}
\end{table}
\end{comment}

\begin{table}
\caption{Statistics of the  benchmark programs in $D_{test}$. 
%B1-B20 are collected
%from~\cite{wang2019mitigating} while B21-B37 are
%originated from~\cite{zhang2018sc}.
}
\vspace{-1em}
\label{tbl:stats}
\centering
\scalebox{0.75}{
\begin{tabular}{|l|c|c|c|c||l|c|c|c|c|}
\hline
Name\ \ \   & LoC   & ${I}_{pub~}$ & ${I}_{priv}$ & ${I}_{rand}$ &
Name\ \ \   & LoC   & ${I}_{pub~}$ & ${I}_{priv}$ & ${I}_{rand}$  \\ \hline\hline
B1  &11    &0   & 2   & 2     & B2  &12     &0  & 2  & 2    \\ \hline
B3  &12    &0   & 1   & 2     & B4  &25     &1  & 1  & 3    \\ \hline
B5  &25    &1   & 1   & 3     & B6  &32     &1  & 1  & 3    \\ \hline
B7  &81    &1   & 1   & 7     & B8  &84     &1  & 1  & 7    \\ \hline
B9  &104   &1   & 1   & 7     & B10 &964    &1  & 16 &32    \\ \hline
B11 &1,130 &1   & 16  & 32    & B12 &1,256  &0  & 25 &75    \\ \hline
B13 &2,506 &0   & 25  & 125   & B14 &3,764  &0  & 25 &175   \\ \hline
B15 &8,810 &0   & 25  & 349   & B16 &13,810 &0  & 25 &575   \\ \hline
B17 &18,858&0   & 25  & 775   & B18 &23,912 &0  & 25 &975   \\ \hline
B19 &30,228&0   & 25  & 1,225 & B20 &34,359 &16 & 16 &1,232 \\ \hline\hline

B21 &79    &0   & 16  & 16    & B22  &67     &0  & 8  &16    \\ \hline
B23 &21    &0   & 2   & 2     & B24   &23     &0  & 2  &2     \\ \hline
B25  &27    &0   & 1   & 2     & B26  &32     &0  & 2  &2     \\ \hline
B27  &40    &0   & 2   & 3     & B28  &59     &0  & 3  &4     \\ \hline
B29  &60    &0   & 3   & 4     & B30 &66     &0  & 3  &4     \\ \hline
B31  &66  &0 & 3 & 4 & B32   &426k       &288   &288    &3205      \\ \hline
B33  &426k      &288    &288     &3205       & B34   &426k       &288   &288    &3205      \\ \hline
B35  &429k      &288    &288     &3205       & B36   &426k      &288   &288    & 3205     \\ \hline
B37  & 442k     &288    &288     & 3205      &    &   &   &    &      \\ \hline
\end{tabular}
}
\vspace{-1em}
\end{table}




\subsection{Performance and Accuracy of the Learned Analyzer}
\label{subsec:analyzer}

%To answer RQ1, 
To demonstrate the advantage of our learned analyzer (answer RQ1),
we compared our learned analyzer with the two existing
tools~\cite{zhang2018sc,wang2019mitigating} on the programs in
$D_{test}$.  Only our analyzer can handle all of the 37 programs (we
encountered errors while running the existing tools on
benchmarks from other source), therefore, we compared the results of our analyzer with
the tool from \cite{wang2019mitigating} on B1-B20, and with the tool
from \cite{zhang2018sc} on B21-B37.  The results are shown in
Table~\ref{tbl:FSE19} and Table~\ref{tbl:CAV18}, respectively.



\begin{table}
\caption{Comparing the learned analyzer with the tool from \cite{wang2019mitigating}. 
%Observe that learned analyzer is
%  consistently faster than the baseline technique, and is almost always just as accurate as the baseline analysis (\# of
%  variables marked UKD and SID).
}
\vspace{-1em}
\label{tbl:FSE19}
\centering
\scalebox{0.73}{
\begin{tabular}{|l|r|c|rrr|c|rrr|}
%\begin{tabular}{|L{0.1\linewidth}|C{0.15\linewidth}|
%                 R{0.15\linewidth}|R{0.1\linewidth}R{0.1\linewidth}R{0.1\linewidth}|
%                 R{0.15\linewidth}|R{0.1\linewidth}R{0.1\linewidth}R{0.1\linewidth}|}
\hline
\multirow{2}{*}{Name}  & \multirow{2}{*}{\# AST}&  \multicolumn{4}{c|}{Manually Designed Analyzer~\cite{wang2019mitigating}} & \multicolumn{4}{c|}{Our Learned Analyzer}   \\\cline{3-10}
       &        &  Time (s) & UKD & SID & RUD    &  Time (s)   & UKD & SID & RUD
\\ \hline\hline
B1     &7      &0.061      &4 &    0 &    22       &\textbf{0.001}     &4 &0 &22
\\ \hline
B2     &6      &0.105      &\textbf{7} &    \textbf{0} &    20       &\textbf{0.001}     &\textbf{6} &\textbf{1} &20
\\ \hline
B3     &8      &0.099      &1 &    3 &    31       &\textbf{0.001}      &1 &3 &31
\\ \hline
B4     &11      &0.208  &\textbf{6}&12&31  &\textbf{0.001}      &\textbf{17}&12&20
\\ \hline
B5     &11      &0.216  &\textbf{1}&10&29  &\textbf{0.001}      &\textbf{11}&10&19
\\ \hline
B6     &14      &0.276  &\textbf{1}&15&48  &\textbf{0.001}      &\textbf{8}&15&41
\\ \hline
B7     &39      &0.213      &2 &    25 &   151      &\textbf{0.002}      &2 &    25 &   151
\\ \hline
B8     &39      &0.147      &4 &    42 &   249      &\textbf{0.002}      &4 &    42 &   249
\\ \hline
B9     &47      &0.266      &2 &   61 &   153      &\textbf{0.001}       &2 &   61 &   153
\\ \hline
B10    &522     &0.550      &31 &    12 &  2334      &\textbf{0.008}      &31 &    12 &  2334
\\ \hline
B11    &522     &0.447      &31&    0 &  2334      &\textbf{0.029}      &31&    0 &  2334
\\ \hline
B12    &426     &0.619      &52 &  300 &  2062      &\textbf{0.001}      &52 &  300 &  2062
\\ \hline
B13    &827     &1.102      &49 &  600 &  4030      &\textbf{0.006}      &49 &  600 &  4030
\\ \hline
B14    &1,228   &1.998      &49 &  900 &  5995      &\textbf{0.065}      &49 &  900 &  5995
\\ \hline
B15    &2,832   &16.999     &49&  2,100 &13861      &\textbf{0.107}      &49&  2,100 &13861
\\ \hline
B16    &4,436   &24.801     &49 &3,300 &21,723     &\textbf{2.663}       &49 &3,300 &21,723
\\ \hline
B17    &6,040   &59.120     &49 &4,500 &29,587      &\textbf{1.956}      &49 &4,500 &29,587
\\ \hline
B18    &7,644   &121.000 %2m1s
                            &47 &5,700 &37,449      &\textbf{3.258}     &47 &5,700 &37,449
\\ \hline
B19    &9,649   &202.000 %3m22s
                            &49 &7200 &47,280      &\textbf{5.381}       &49 &7200 &47,280
\\ \hline
B20    &13,826  &972.000 %16m12s
                            &127 &26,330 &38,070      &\textbf{3.650}    &127 &26,330 &38,070
\\ \hline
\end{tabular}
}
\vspace{-.5em}
\end{table}



In both tables, Columns~1-2 show the benchmark name and the number of
AST nodes.  Columns~3-6 show the existing tool's analysis time and
result, including a breakdown in the three types.  Similarly,
Columns~7-10 show our learned analyzer's time and result.
%
%
Note that in~\cite{wang2019mitigating}, the $\UKD$/$\SID$/$\RUD$ numbers they
collected were the number of variables of the LLVM IR, and thus larger
than the number of variables in the original programs. To be
consistent, we compared with their results in the same manner in
Table~\ref{tbl:FSE19}.

% 1. we firstly talk about the speed  compared with [1]
% 2. we then talk about the speed  compared with [2]
% 3. then we talk about the accuracy
Table~\ref{tbl:FSE19} and Table~\ref{tbl:CAV18} contain
the results of comparing our tool with the state-of-the-art tools~%
\cite{wang2019mitigating} and~\cite{zhang2018sc} respectively,
where our learned analyzer is much faster, especially on 
larger programs such as B20 (3.6 seconds versus 16 minutes).
\textcolor{red}{The reason why our analyzer is faster is because the manually-crafted analyses
~\cite{wang2019mitigating,zhang2018sc}
rely on evaluating set-relations (e.g. difference and intersection 
of sets of random variables), 
whereas our DSL syntax is designed without set operations to infer 
the same types, thus leading to a faster analysis.}
Although in general the set operation-based algorithm is
more accurate, it has an extremely large computational overhead.
Moreover, in practice, it does not always improve precision.
\textcolor{red}{
Furthermore, the method in \cite{zhang2018sc} uses an SMT solver
based model counting technique to infer leak-free variables,
 which is significantly more expensive than type inference. 
}
%This is because our analyzer relies on simpler inference rules,
%whereas the existing tool~\cite{wang2019mitigating} relies on the more
%complex set-theoretic operations (difference and intersection of sets of random
%variables). Although in principle the set operation-based algorithm could be 
%more accurate, it had large computational overhead.
%Moreover, in practice, it did not always improve the accuracy. 
%
%

% 2. then we talk about the accuracy
% 2.1 What does accuracy mean here?
% 2.2 Why our tool achieves almost same as manual analysis?
% 2.3 Why our tool fails in some cases?
% 2.4 Why our tool also does better on some cases?
As shown in Table~\ref{tbl:FSE19} and Table~\ref{tbl:CAV18}, 
by learning inference rules from data, we can achieve almost the same 
accuracy as manual analysis~\cite{wang2019mitigating,zhang2018sc} 
while avoiding the huge overhead.
\textcolor{red}{
Given the same definitions of distribution types
($\UKD$, $\SID$ and $\RUD$), both our learned rules and
manual analysis rules~\cite{wang2019mitigating,zhang2018sc} 
 can infer the non-leaky patterns,  thus recognizing the variable 
 types correctly under most benchmarks in
Table~\ref{tbl:FSE19} and Table~\ref{tbl:CAV18},}
%
except for B4-B6 and B30, where set operations are required to prove
the leak-freedom of some variables.
 Recall that losing accuracy here
indicates that our learned rules infer the types more conservatively,
without losing soundness.
%
Nevertheless, our analyzer also increased accuracy in some other cases
(e.g., B2), due to its deeper constant propagation (which led to the
proof of more $\SID$ variables) while the existing
tool~\cite{wang2019mitigating} failed to do so, and conservatively
marked them as $\UKD$ variables.


\begin{comment}
For B4-B6, our analyzer missed the following three inference rules for
random variable $x$:
\begin{center}
$\exists$ $x_1$, $x_2$ $f$($x$, $x_1$) $\wedge$ $f$($x$, $x_2$)
$\wedge$ $x_1$=$x_2$ $\wedge$ \\
$\mathbb{INRAND}$($x_1$) $\wedge$ $\mathbb{INRAND}$($x_2$) $\rightarrow$ ${\phi}_1$($x$) \\
$\exists$ $x_1$ $\forall x_2$, $f$($x$, $x_1$) $\wedge$ $f$($x$, $x_2$)
$\wedge$ $x_1 \neq x_2$ $\wedge$ \\
$\mathbb{INRAND}$($x_1$) $\wedge$ $\mathbb{INRAND}$($x_2$) $\rightarrow$ ${\phi}_2$($x$) \\
\end{center}
%
%Here, the SyGuS synthesized relation $f$($x$, $x_1$) means that, in
%%the AST, there is a path from input $x_1$ to intermediate node $x$;
%and if ${\phi}_1$($x$) $\wedge$ ${\phi}_2$($x$) holds, $x$ is
%classified as RUD.

However, in Datalog, the variable bounded in the rule body is
existentially quantified.  To to express universal quantification,
negation is needed.  Unfortunately, our SyGuS grammar $\mathcal{L}_f$
does not allow negation in the IDB predicates.
%
The tool from \cite{wang2019mitigating}, on the other hand, defines
$f$($x$, $S$) where $S$ represents a set and uses the (expensive)
set operations to replace the universal quantification.
%
Thus, they have chosen to gain accuracy in some rare cases by paying
for a significant slowdown in most cases.
\end{comment}




\begin{table}
\caption{Comparing the learned analyzer with SCInfer~\cite{zhang2018sc}.}
\vspace{-1em}
\label{tbl:CAV18}
\centering
\scalebox{0.75}{
\begin{tabular}{|l|r|c|rrr|c|rrr|}\hline
%\begin{tabular}{|L{0.1\linewidth}|C{0.15\linewidth}|
 %                R{0.15\linewidth}|R{0.1\linewidth}R{0.1\linewidth}R{0.1\linewidth}|
 %                R{0.15\linewidth}|R{0.1\linewidth}R{0.1\linewidth}R{0.1\linewidth}|}
\hline
\multirow{2}{*}{Name} & \multirow{2}{*}{\# AST}  & \multicolumn{4}{c|}{The SCInfer Verification Tool~\cite{zhang2018sc}} & \multicolumn{4}{c|}{Our Learned Analyzer}
\\\cline{3-10}
    &      & Time (s)  & UKD&SID&RUD          &  Time (s)   & UKD&SID&RUD
\\ \hline\hline
B21  &32   & 0.390     & 16&0&16        & \textbf{0.005}      & 16&0&16
\\ \hline
B22  &24   & 0.570     & 8&0&16         & \textbf{0.002}      & 8&0&16
\\ \hline
B23  &6    & 0.010     & 0&0&6          & \textbf{0.001}      & 0&0&6
\\ \hline
B24  &6    & 0.060     & 0&0&6          & \textbf{0.001}      & 0&0&6
\\ \hline
B25  &8    & 0.250     & 0&2&6          & \textbf{0.001}      & 0&2&6
\\ \hline
B26  &9    & 0.160     & 2&3&4          & \textbf{0.002}      & 2&3&4
\\ \hline
B27  &11   & 0.260     & 1&5&5          & \textbf{0.001}      & 1&5&5
\\ \hline
B28  &18   & 0.290     & 3&4&11         & \textbf{0.003}      & 3&4&11
\\ \hline
B29  &18   & 0.230     & 2&4&11         & \textbf{0.002}      & 2&4&12
\\ \hline
B30  &28   & 0.340     & 2&6&20         & \textbf{0.001}      & \textbf{8}&0&20
\\ \hline
B31  &28   & 0.500     & 2&7&19         & \textbf{0.001}      & 2&7&19
\\ \hline
B32  &197k & 3.800     & 0&6.4k&190.4k  & \textbf{3.180}          & 0&6.4k&190.4k
\\ \hline
B33  &197k & 2,828.000 %47m8s
                       & 4.8k&6.4k&185.6k  & \textbf{3.260}         & 4.8k&6.4k&185.6k
\\ \hline
B34  &197k & 2,828.000 %47m8s
                       & 3.2k&6.4k&187.2k  & \textbf{3.170}          & 3.2k&6.4k&187.2k
\\ \hline
B35  &198k & 2,828.000 %47m8s
                       & 1.6k&8k&188.8k  & \textbf{3.140}          &\textbf{3.2k}&8k&187.2k
\\ \hline
B36  &197k & 2,828.000 %47m8s
                       & 4.8k&6.4k&185.6k  & \textbf{3.150}           & 4.8k&6.4k&185.6k
\\ \hline
B37  &205k & 2,828.000 %47m8s
                       & 17.6k&1.6k&185.6k  & \textbf{3.820}         & 17.6k&1.6k&185.6k
\\ \hline
\end{tabular}
}
\vspace{-1em}
\end{table}



%Table~\ref{tbl:CAV18} shows the results of comparing our learned analyzer with
%SCInfer~\cite{zhang2018sc}, which relies on SMT solver
%based \emph{model counting} techniques to decide
%whether a variable is leak-free.  However, model counting is computationally 
% more expensive than type inference.  Our
%results in Table~\ref{tbl:CAV18} show that, again, our learned analyzer achieves almost the
%same accuracy while being several orders-of-magnitude faster than SCInfer.
%
\subsection{Effectiveness of Rule Induction and Soundness Verification}
\label{subsec:learnerProver}


To answer RQ2 and RQ3, we collected statistics while applying \GPS{}
to the 531 small programs in $D_{test}$, as shown in 
Table~\ref{tbl:result-learning}.  In total, \GPS{}
took 30 iterations to complete the entire learning process.
%
Column 1 shows the iteration number and Column 2 shows the time taken
by the \emph{learner} and the \emph{prover} together.  Columns~3-6
show the number of inference rules learned during the iteration,
together with their types ($\UKD$, $\SID$, and $\RUD$).
%
Similarly, Columns~7-10 show the number of verified inference rules.


The next two columns show the following statistics: (1) the size of
the learned decision tree (\# Tree$_{learn}$) in terms of the number
of decision nodes; (2) the number of counter-examples (CEX) added by
the prover (\# AST$_{CEX}$); they are added to the 531 original
training programs before the next iteration starts.
%
The last column shows the number of features generated by SyGuS; these
features are added to the original feature set and then used by the
learner during the next iteration.


\begin{table*}
\caption{Decision Tree Learning with Feature Synthesis (Different Iterations with \#AST = 531).}
\vspace{-1em}
\label{tbl:result-learning}
\centering
\scalebox{0.73}{
\begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Iteration}  
& \multirow{2}{*}{Time (s) } 
%& \multirow{2}{*}{$\#{Rule}_{learned}$}
& \multicolumn{4}{c|}{\# Rules Learned}
%& \multirow{2}{*}{$\#{Rule}_{verified}$}
& \multicolumn{4}{c|}{\# Rules Verified}
& \multirow{2}{*}{\# Tree$_{learn}$}
& \multirow{2}{*}{\# AST$_{CEX}$} 
& \multirow{2}{*}{\# Feature$_{syn}$}   
\\\cline{3-6} \cline{7-10}

    &   & \ \ \ Total\ \ \  & \textit{UKD}  &\textit{SID}  &\textit{RUD}  
        & \ \ \ Total\ \ \  & \textit{UKD}  &\textit{SID}  &\textit{RUD}  
        &  & &
\\\hline\hline
  1 & 1.316 & 9  & 2 & 2 & 5 & 5 & 2 & 1& 2 & 23 & 4 & 5
 \\\hline
  2 & 0.775 & 8  & 2 & 2 & 4 & 4 & 2 & 1& 1 & 17 & 9 & 7
  \\\hline
  3 & 1.115 & 8  & 2 & 2 & 4 & 5 & 2 & 2 & 1 & 24 & 13 & 9
 \\\hline
  4 & 0.511 & 8  & 2 & 2 & 4 & 5 & 2 & 1 & 2 & 18 & 18 & 10
 \\\hline
  5 & 0.513 & 8  & 2 & 2 & 4 & 7 & 2 & 2 & 3 & 27 & 21 & 11
 \\\hline
  6 & 0.537 & 8  & 2 & 2 & 4 & 6 & 2 & 2 & 2 & 24 & 25 & 12
 \\\hline
  7 & 0.510 & 8  & 2 & 2 & 4 & 6 & 2 & 2 & 2 & 26 & 29 & 13
 \\\hline
  8 & 0.512 & 8  & 2 & 2 & 4 & 6 & 2 & 2 & 2 & 28 & 33 & 14
 \\\hline
  9 & 0.511 & 8  & 2 & 2 & 4 & 6 & 2 & 2 & 2 & 30 & 37 & 15
 \\\hline
  10 & 0.524 & 8  & 2 & 2 & 4 & 5 & 2 & 2 & 1 & 32 & 41 & 16
  \\\hline
  11 & 0.546 & 8  & 2 & 2 & 4 & 4 & 2 & 2 & 0 & 34 & 45 & 17
  \\\hline
  12 & 0.556 & 8  & 2 & 2 & 4 & 4 & 2 & 2 & 0 & 36 & 49 & 18
  \\\hline
  13 & 0.550 & 8  & 2 & 2 & 4 & 5 & 2 & 2 & 1 & 38 & 53 & 19
  \\\hline
  14 & 0.540 & 8  & 2 & 2 & 4 & 6 & 2 & 2 & 2 & 40 & 57 & 20
  \\\hline
  15 & 0.542 & 8  & 2 & 2 & 4 & 4 & 2 & 2 & 0 & 42 & 61 & 21
  \\\hline
  16 & 0.552 & 8  & 2 & 2 & 4 & 6 & 2 & 2 & 2 & 44 & 65 & 22
  \\\hline
  17 & 0.577 & 8  & 2 & 2 & 4 & 5 & 2 & 2 & 1 & 46 & 69 & 23
  \\\hline
  18 & 0.598 & 8  & 2 & 2 & 4 & 6  & 2 & 2 & 2 & 48 & 73 & 24
  \\\hline
  19 & 0.571 & 8  & 2 & 2 & 4 & 6 & 2 & 2 & 2 & 50 & 77 & 25
  \\\hline
  20 & 0.673 & 8  & 2 & 2 & 4 & 5 & 1 & 2 & 2 & 52 & 82 & 26
  \\\hline
  21 & 0.526 & 8  & 2 & 2 & 4 & 3 & 1 & 2 & 0 & 54 & 87 & 27
  \\\hline
  22 & 0.525 & 8  & 3 & 2 & 3 & 6  & 3 & 2 & 1 & 35 & 91 & 27
  \\\hline
  23 & 0.697 & 9  & 3 & 2 & 4 & 7 & 2 & 2 & 3 & 37 & 93 & 27
  \\\hline
  24 & 0.700 & 9  & 3 & 2 & 4 & 8 & 2 & 2 & 4 & 38 & 95 & 28
  \\\hline
  25 & 0.691 & 7  & 2 & 2 & 3 & 6 & 1 & 2 & 3 & 36 & 97 & 29
  \\\hline
  26 & 0.707 & 7  & 2 & 2 & 3 & 6 & 1 & 2 & 3 & 37 & 99 & 30
  \\\hline
  27 & 0.716 & 7  & 2 & 2 & 3 & 6 & 1 & 2 & 3 & 38 & 101 & 31
  \\\hline
  28 & 0.540 & 7  & 2 & 2 & 3 & 6 & 1 & 2 & 3 &  39 & 102 & 32
  \\\hline
  29 & 0.534 & 7  & 2 & 2 & 3 & 6 & 1 & 2 & 3 & 39 & 103 & 32
  \\\hline
  30 & 0.528 & 7  & 2 & 2 & 3 & 7 & 2 & 2 & 3 & 39 & 104 & 32
  \\\hline\hline
TOTAL & 18.693 & 237 & 63 & 60 & 114 & 167 & 54 & 57 & 56 & 1071 & 1833 & 622
  \\\hline
\end{tabular}
}
\vspace{-1em}
\end{table*}







The results demonstrate the efficiency of both the learner and the prover.
%; together, the 30 iterations over 531 training
%examples finished in 18 seconds.
%
%
Within the \emph{learner}, the number of rules produced in each
iteration remains modest (8 on average), indicating it has
successfully avoided overfitting.
%
%
\textcolor{red}{
%
This is because the SyGuS solver is biased towards producing small features which, by Occam's razor, are likely to generalize well. 
%Our experimental results also showed that the amount of the learned rules were small (8 rules with respect to 531 AST examples), which indicates that overfitting was unlikely.
%
Furthermore, any learned analysis rules have to pass the soundness check, and this provides additional assurance against overfitting to the training data.
%
%Finally, we have inspected the synthesized features and inference rules, and found that they are generally-applicable (i.e., not specific to any individual program structure), and they are broadly similar to the rules we have shown in Example IV.1.
}  
%
%
The \emph{prover} either quickly verifies a rule, or quickly drops after
adding a counter-example to prevent it from being learned again.
%After
%30 iterations, a total of 104 such counter-examples have been added.
%
In early iterations, about half of all learned rules can be proved,
but as more counter-examples are added, the quality of the learned
rules improves, and thus the percentage of proved rules also increases.


\textcolor{red}{
\subsection{Threats to Validity}
}

\textcolor{red}{
%
Our experimental evaluation focused on cryptographic software, which
is structurally simple and, unlike general-purpose software, does not
exercise complicated language constructs (data-dependent loop bounds,
recursion, non-termination, etc.). It is an interesting direction of
future work to extend our techniques to these more general classes of
software code.
%
}

\textcolor{red}{
%
A notable limitation in our work is the assumption of the knowledge
base (KB). While the KB is readily available for our application domain
(side-channel analysis), for other applications, it might be
non-trivial to construct. Furthermore, an
incorrect KB might compromise the soundness of the learned rules,
although in this work, we have carefully mitigated this threat by
curating the proof rules from previous
papers~\cite{zhang2018sc,eldib2014synthesis,barthe2015verified} that
have themselves formally verified the validity of these proof rules.
%
}

\vspace{2ex}


==> frontmatter.tex <==
\IEEEoverridecommandlockouts
% The preceding line is only needed to identify funding in the first footnote. If that is unneeded, please comment it out.

==> images/learner/AST.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% b2 = i2 xor r2
% b3 = i3 xor r3
% b4 = b2 xor b3

\begin{tikzpicture}[
  font=\scriptsize,
  level 1/.style={sibling distance=25mm},
  level 2/.style={sibling distance=15mm},
  level distance = 2em,
]

  \node [root, label=right:{\lstinline|b4|}] {$\oplus$}
  child {
    node [root, label=right:{\lstinline|b2|}] {$\oplus$}
    child {
      node [env] {\lstinline|i2|}
      edge from parent
    } child {
      node [env] {\lstinline|r2|}
      edge from parent
    }
    edge from parent
  } child {
    node [root, label=right:{\lstinline|b3|}] {$\oplus$}
    child {
      node [env] {\lstinline|i3|}
      edge from parent
    } child {
      node [env] {\lstinline|r3|}
      edge from parent
    }
    edge from parent
  };

\end{tikzpicture}

\vspace{2em}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% n4 = b2 or b3

\begin{tikzpicture}[
  font=\scriptsize,
  level 1/.style={sibling distance=25mm},
  level 2/.style={sibling distance=15mm},
  level distance = 2em,
]

  \node [root, label=right:{\lstinline|n4|}] {$\lor$}
  child {
    node [root, label=right:{\lstinline|b2|}] {$\oplus$}
    child {
      node [env] {\lstinline|i2|}
      edge from parent
    } child {
      node [env] {\lstinline|r2|}
      edge from parent
    }
    edge from parent
  } child {
    node [root, label=right:{\lstinline|b3|}] {$\oplus$}
    child {
      node [env] {\lstinline|i3|}
      edge from parent
    } child {
      node [env] {\lstinline|r3|}
      edge from parent
    }
    edge from parent
  };

\end{tikzpicture}


==> images/learner/rudRule.tex <==
%\documentclass[border=10pt]{standalone}
%\usepackage{tikz}

%\begin{document}
\begin{tikzpicture}[font=\scriptsize] 
  [
    grow                    = right,
    sibling distance        = 8em,
    level distance          = 2em,
    edge from parent/.style = {draw, -latex},
    every node/.style       = {font=\footnotesize},
    sloped
  ]
  %%%%%% First Decision Tree
  \node [root] at (-1.8, 0) {$\oplus$}  % t7
  child{ node [root] at (-.1, .7) {$\land$}  % t1
   child{node [env] at (-.1, .7)  {$r1$} 
   edge from parent node  [above, align=center]{}
   }
   child{
   node [env] at (-.5, .7)  {$key$}
   edge from parent node  [above, align=center]{}
   }
  edge from parent node  [above, align=center]{}
  }
  child{ node [root] at (.1, .7) {$\oplus$}  % t4
   child{node [env] at (.2, .7)  {$r2$} 
   edge from parent node  [above, align=center]{}
   }
   child{ node [env] at (.1, .7)  {$b$}
   edge from parent node  [above, align=center]{}
   }
   edge from parent node  [above, align=center]{}
  };
  
    \node [root] at (2.3, 0) {$\oplus$}  % t6
  child{ node [root] at (-.1, .7) {$\oplus$}  % t3
   child{node [env] at (-.1, .7)  {$key$} 
   edge from parent node  [above, align=center]{}
   }
   child{
   node [env] at (.1, .7)  {$r2$}
   edge from parent node  [above, align=center]{}
   }
  edge from parent node  [above, align=center]{}
  }
  child{ node [root] at (.1, .7) {$\oplus$}  % t2
   child{node [env] at (-.1, .7)  {$r2$} 
   edge from parent node  [above, align=center]{}
   }
   child{ node [env] at (.1, .7)  {$b$}
   edge from parent node  [above, align=center]{}
   }
   edge from parent node  [above, align=center]{}
  };
  
  %%%%%% add text
  
  \node[minimum width=18mm, minimum height=6mm, dashed, draw=black, thick, align=center] (PR1) at (-2.1, 0) {};
   \node[minimum width=18mm, minimum height=6mm, dashed, draw=black, thick, align=center] (PR1) at (2, 0) {};
  \node at (-1.4,0) {$t7$};
  \node at (-2.5,0) {$\lnot h(t7)$};
  \node at (-3.4,0) {$\mathbb{RUD}$};
  %\node at (-2.2,-.8) {$t3$};
  \node at (-3.4,-.8) {$g(L,r1)$};
  %\node at (-.5,-.8) {$t2$};
  \node at (-1.8,-.8) {$g(R,r2)$};
   \node at (2.7,0) {$t5$};
   \node at (1.6,0) {$h(t5)$};
   \node at (.7,0) {$\textcolor{red}{\mathbb{UKD}}$};
  % \node at (1.9,-.8) {$t3$};
   \node at (.7,-.8) {$g(L,r2)$};
  % \node at (3.6,-.8) {$t4$};
   \node at (2.4,-.8) {$g(R,r2)$};
   \node at (-3.8,-2.1) {$g(r1,r1)$};
   \node at (-1.5,-2.1) {$g(r2,r2)$};
   \node at (2.4,-2.1) {$g(r2,r2)$};
\end{tikzpicture}
%\end{document}


==> images/overall/overall.tex <==
\begin{algorithmic}[1]
\Input Examples, $\mathcal{E} = \{ (x_1, \TYPE(x_1)), (x_2, \TYPE(x_2)), \dots, (x_n, \TYPE(x_n)) \}$
\Input Features, $\mathcal{F} = \{ f_1, f_2, \dots, f_k \}$
\Output $Analyzer$

\State $bound$: the upper bound of iteration times

\For {$i \in \{ 1, 2, 3, \dots, bound \}$}
  \State $A_i = DTL(\mathcal{E}, \mathcal{F})$
  \State $R_{rej} = \textsc{Prover}(A_i)$
  \If {$R_{rej} = \emptyset$}
    \State \textbf{return} $\textsc{Select}(\Phi)$
  \Else
    \State $\mathcal{E}_{\alpha} = genCounterExample(\mathcal{E}, \mathcal{F}, R_{rej})$
    \State $\mathcal{E} = \mathcal{E} \union \mathcal{E}_{\alpha}$
  \EndIf
\EndFor

\State \textbf{return} $\emptyset$
\end{algorithmic}

% \algsetup{linenosize=\tiny}
% \footnotesize
% \begin{algorithmic}[1]
% \STATE \textbf{Input:} Examples $\mathcal{E}$, Features $\mathcal{F}$
% \STATE \textbf{Output:} $Analyzer$  \\
% \STATE $bound$: the upper bound of iteration times \\
%   \For{iteration $i$ from 1 till $bound$}
% {
% 	\STATE $A_i$ = $DTL$($\mathcal{E}$, $\mathcal{F}$) \\
% 	\STATE $R_{rej}$ = $Prover$($A_i$)\\
% 	\STATE \textbf{if} $R_{rej}$ = $\emptyset$ \Return $A_i$
% 	\STATE \textbf{else} $\mathcal{E}_{\alpha}$ = $genCounterExample$($\mathcal{E}$, $\mathcal{F}$, $R_{rej}$)
% 	\STATE $\mathcal{E}$ = $\mathcal{E} \cup \mathcal{E}_{\alpha}$
% }
% \Return $\emptyset$
% \end{algorithmic}


==> images/prover/cex.tex <==
\begin{algorithmic}[1]
\Input Examples, $\mathcal{E} = \{ (x_1, \TYPE(x_1)), (x_2, \TYPE(x_2)), \dots, (x_n, \TYPE(x_n)) \}$
\Input Features, $\mathcal{F} = \{ f_1, f_2, \dots, f_k \}$
\Output $Analyzer$

\State $bound$: the upper bound of iteration times

\For {$i \in \{ 1, 2, 3, \dots, bound \}$}
  \State $A_i = DTL(\mathcal{E}, \mathcal{F})$
  \State $R_{rej} = \textsc{Prover}(A_i)$
  \State ${acc}_i = \textsc{Cal}\textsc{Accuracy}(A_{i} / R_{ref}, \mathcal{E})$
  \State $\Phi = \Phi \union \textsc{Store}(acc_i, A_i / R_{ref})$
  \If {$R_{rej} = \emptyset$}
    \State \textbf{return} $\textsc{Select}(\Phi)$
  \Else
    \State $\mathcal{E}_{\alpha} = genCounterExample(\mathcal{E}, \mathcal{F}, R_{rej})$
    \State $\mathcal{E} = \mathcal{E} \union \mathcal{E}_{\alpha}$
  \EndIf
\EndFor

\State \textbf{return} $\textsc{Select}(\Phi)$
\end{algorithmic}

% \algsetup{linenosize=\tiny}
% \footnotesize
% \begin{algorithmic}[1]
% \STATE \textbf{Input:} Examples $\mathcal{E}$, Features $\mathcal{F}$
% \STATE \textbf{Output:} $Analyzer$  \\
% \STATE $bound$: the upper bound of iteration times \\
%   \For{iteration $i$ from 1 till $bound$}
% {
% 	\STATE $A_i$ = $DTL$($\mathcal{E}$, $\mathcal{F}$) \\
% 	\STATE $R_{rej}$ = \textsc{Prover}($A_i$)\\
% 	\STATE ${acc}_i$ = \textsc{Cal}\textsc{Accuracy}($A_{i}/R_{rej}, \mathcal{E}$)  \\
% 	\STATE $\Phi$ = $\Phi$ $\cup$ \textsc{Store}($acc_i, A_{i}/R_{rej}$) \\
% 	\STATE \textbf{if} $R_{rej}$ = $\emptyset$ \Return \textsc{Select}($\Phi$)\\
% 	\STATE \textbf{else} $\mathcal{E}_{\alpha}$ = $genCounterExample$($\mathcal{E}$, $\mathcal{F}$, $R_{rej}$)
% 	\STATE $\mathcal{E}$ = $\mathcal{E} \cup \mathcal{E}_{\alpha}$
% }
% \Return \textsc{Select}($\Phi$)
% \end{algorithmic}


==> images/prover/select.tex <==
\begin{algorithmic}[1]
\Input Tuple set $\Phi$ with $<acc, R>$
\Output $Analyzer$

\State $\Phi_s = \textsc{Sorted}(\Phi, key=\lambda x: x[0], reverse=True)$
\State \textbf{return} ${\Phi}_s[0][1]$
\end{algorithmic}

% \algsetup{linenosize=\tiny}
% \footnotesize
% \begin{algorithmic}[1]
% \STATE \textbf{Input:} Tuple Set $\Phi$ with <$acc, R$>
% \STATE \textbf{Output:} $Analyzer$  \\
% \STATE ${\Phi}_s$ = \textsc{Sorted}( $\Phi$, $key=\lambda x: x[0]$, reverse=True )\\
% \Return ${\Phi}_s$[0][1];
% \end{algorithmic}


==> introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Static analyses are being increasingly used to detect security
vulnerabilities such as \emph{side channels}~\cite{wang2019mitigating,
  zhang2018sc,chen2017precise,brennan2018symbolic}.
However, manually crafting a static analyzer to balance between
accuracy and efficiency is not an easy task: even for domain experts,
it can be labor intensive, error prone, and result in suboptimal
implementations.
%
For example, we may be tempted to add expensive analysis rules for
specific sanitized patterns without realizing they are rare in target
programs.  Even if the analysis rules are carefully tuned to a corpus
of code initially, they are unresponsive to changing characteristics
of the target programs and thus may become suboptimal over time;
manually updating them to keep up with the new programs would be
difficult.


One way to make better accuracy-efficiency trade-offs and to
dynamically respond to the distribution of target programs is to use
data-driven approaches~\cite{bielik2017learning,mendis2019compiler}
that automatically synthesize analyses from labeled examples provided
by the user.  However, checking soundness or compliance with user
intent (generalization) has always formed a significant challenge for
example-based synthesis techniques~\cite{gulwani2012spreadsheet,
  leung2015interactive, singh2012synthesizing, smith2016mapreduce,
  solar2006combinatorial}.  The lack of soundness guarantees, in
particular, hinders the application of such learned analyzers in
security-critical applications. While several existing
works~\cite{an2019augmented, mayer2015user, singh2015predicting,
  devlin2017robustfill} try to address this problem, rigorous
soundness guarantees have remained elusive.


To overcome this problem, we propose a learning-based method for 
synthesizing a
\emph{provably-sound} static analyzer that detects side channels
in cryptographic software, by inferring a
\emph{distribution} type for each program variable that indicates
if its value is statistically dependent on the secret.
%
The overall flow of our method, named \GPS{}, is shown in
Fig.~\ref{overview}. The input is a set of training data and the
output is a learned analyzer.  The training data are small programs
annotated with the ground truth, e.g., which program variables have
leaks.




\setlength{\textfloatsep}{10pt plus 1.0pt minus 2.0pt}
\begin{figure}
\centering
\scalebox{0.85}{\input{images/introduction/jigsaw.tex}}
\caption{The overall flow of \GPS{}, our data-driven synthesis method.}
\label{overview}
\end{figure}



Internally, \GPS{} consists of \emph{learner} and \emph{prover}.
%
The \emph{learner} uses syntax guided synthesis (SyGuS) to generate
recursive features and decision tree learning (DTL) to generate type-inference
rules based on these features; it returns a set $R$ of Datalog
formulas that codify these rules.
%%%%%%%%%
%The \emph{prover} checks if the rules are valid by solving a \emph{query containment checking} problem, i.e., each rule must be justified by some existing proof rules called the knowledge base ($KB$).
%%%%%%%%
The \emph{prover} checks the soundness of each learned rule, i.e., it is not only consistent with the training examples but also valid for any other unseen programs. This is formulated by solving a \emph{query containment checking} problem, i.e., each rule must be justified by existing proof rules called the knowledge base ($KB$).
%%%%%%%%%%%
Since only proved rules are added to the analyzer, the analyzer is guaranteed to be sound. If a rule cannot be proved, we add a counter-example to prevent the \emph{learner} from generating it again. 
%
%Soundness is guaranteed because only proved rules are added to the analyzer. If a rule cannot be proved, we add a counter-example to prevent the \emph{learner} from generating it again.

We have implemented \GPS{} in LLVM and evaluated it on 568 programs
that implement cryptographic protocols and
algorithms~\cite{barthe2015verified,blomer2004provably,bayrak2013sleuth}.
Together, they have 2,691K lines of C code.  We compared our learned
analyzer with two state-of-the-art, hand-crafted side-channel analysis
tools~\cite{zhang2018sc,wang2019mitigating}.
%
Our experiments show that the learned analyzer achieves the same
empirical accuracy as the two state-of-the-art tools, while being
several orders-of-magnitude faster.  Specifically, \GPS{} is, on
average, 300$\times$ faster than the analyzer from
\cite{wang2019mitigating} and 900$\times$ faster than the analyzer
from \cite{zhang2018sc}.


To summarize, this paper makes the following contributions:
\begin{itemize}
\item
We propose a data-driven method for learning a provably sound static
analyzer using syntax guided synthesis (SyGuS) and decision tree
learning (DTL).
\item
We guarantee soundness by formulating and solving a Datalog query
containment checking problem.
\item
We demonstrate the effectiveness of our method for
detecting side channels in cryptographic software.
\end{itemize}



%%%%%%%%%%%%%%%%%%%%


In the remainder of this paper, we begin by presenting the 
\textcolor{red}{technical background in Section~\ref{sec:prelims} and our motivating
example in Section~\ref{sec:motivation}.}
We then describe the \emph{learner} in
Section~\ref{sec:learner} and the \emph{prover} in
Section~\ref{sec:prover}, followed by the experimental results in
Section~\ref{sec:experiment}.  
Finally, we survey the related work in
Section~\ref{sec:related} and conclude in
Section~\ref{sec:conclusion}.


==> kb_distribution.tex <==
\begin{figure*}
{\footnotesize
\begin{mathpar}
{\footnotesize
\inferrule*[right=($D_{1.1}$)]{\Gamma \vdash x : \INRANDOP}{supp(x, \{x\} )} \hspace{4ex}
\inferrule*[right=($D_{1.2}$)]{\Gamma \vdash x : \INKEYOP}{supp\text{(}x, \{x\} \text{)}} \hspace{4ex}
\inferrule*[right=($D_{1.3}$)]{\Gamma \vdash x : \INPUBOP}{supp\text{(}x, \{x\} \text{)}} \hspace{4ex}
\inferrule*[right=($D_{2.1}$)]{\Gamma \vdash x : \INRANDOP}{dom(x, \{x\})} \hspace{3ex}
\inferrule*[right=($D_{2.2}$)]{\Gamma \vdash x : \INKEYOP}{dom(x, \emptyset)}
}
\end{mathpar}
\begin{mathpar}
{\footnotesize
\inferrule*[right=($D_{1.4}$)]{\Gamma \vdash x,y : \mathsf{v},~ \Gamma \vdash S : \mathsf{Set}~\mathsf{v}, \RCOP (y, x_1) \wedge \LCOP ( y, x_2 ) \wedge supp(x_1, S_{1}) \wedge supp(x_2, S_{2})}{supp(y, S_1\cup S_2)} \hspace{10ex}
\inferrule*[right=($D_{2.3}$)]{\Gamma \vdash x : \INPUBOP}{dom\text{(}x, \emptyset \text{)}} 
}
\end{mathpar}
\begin{mathpar}
{\footnotesize
\inferrule*[right=($D_{2.4}$)]{\Gamma \vdash x,y : \mathsf{v}, \Gamma \vdash S : \mathsf{Set}~\mathsf{v},  \RCOP ( y, x_1 ) \wedge \LCOP ( y, x_2 ) \wedge \XOROP ( y ) \wedge dom(x_1, S_{1}) \wedge dom(x_2, S_{2})}{dom(x, (S_1 \cup S_2 )/(S_1 \cap S_2 ))}
}
\end{mathpar}
\begin{mathpar}
{\footnotesize
\inferrule*[right=($D_{3}$)]{\Gamma \vdash x : \mathsf{v}, \Gamma \vdash S : \mathsf{Set}~\mathsf{v}, dom(x, S_{x}) \wedge S_{x} \neq \emptyset}{\Gamma \vdash x : \RUD} \hspace{10ex}
\inferrule*[right=($D_{4}$)]{\Gamma \vdash x : \INKEYOP, \Gamma \vdash S :  \mathsf{Set}~\INKEYOP}{\Gamma \vdash x :: S : \mathsf{Set}~\INKEYOP} 
%\inferrule*[right=($D_{5}$)]{\Gamma \vdash x : \mathsf{v}, S : \mathsf{Set}~\mathsf{v}, S_k : \mathsf{Set}~\mathbb{INKEY}, dom\text{(}x, S_{d}\text{)} \wedge S_{d} \text{=} \emptyset \wedge supp\text{(}x, S_{s}\text{)} \wedge S_{s} \cap S_k \text{=} \emptyset}{\mathbb{SID} \text{(} x\text{)}} \and
}
\end{mathpar}
\begin{mathpar}
{\footnotesize
\inferrule*[right=($D_{5}$)]{\inferrule{\Gamma \vdash x : \mathsf{v},~ \Gamma \vdash S_k : \mathsf{Set}~\INKEYOP, ~\\\\~ \Gamma \vdash S_d : \mathsf{Set}~\RUD,~ \Gamma \vdash S_s : \mathsf{Set}~\mathsf{v},~\\\\~ dom(x, S_{d}) \wedge S_{d} \text{=} \emptyset  \wedge supp(x, S_{s}) \wedge S_{s} \cap S_k \text{=} \emptyset}{} }{\Gamma \vdash x : \SID} \hspace{10ex}
\inferrule*[right=($D_{6}$)]{\inferrule {\Gamma \vdash x_1 : \SID,~\Gamma \vdash x_2 : \RUD,~\Gamma \vdash S_1, S_2 : \mathsf{Set}~\mathsf{v}~ \\\\ \LCOP ( y, x_1 ) \wedge \RCOP( y, x_2) \wedge \ANDOP ( y ) ~ \\\\ \wedge supp (x_1, S_1) \wedge supp (x_2, S_2) \wedge S_1 \cap S_2 \text{=} \emptyset}{} }{\Gamma \vdash y : \SID}
}
\end{mathpar}
\begin{mathpar}
{\footnotesize
\inferrule*[right=($D_{7}$)]{\inferrule {\Gamma \vdash x_1 : \SID,~\Gamma \vdash x_2 : \RUD,~\Gamma \vdash S_1, S_2 : \mathsf{Set}~\mathsf{v}~ \\\\  \LCOP ( y, x_1 ) \wedge \RCOP ( y, x_2) \wedge \OROP ( y ) \wedge \\\\ supp (x_1, S_1 ) \wedge supp (x_2, S_2) \wedge S_1 \cap S_2 \text{=} \emptyset}{} }{\Gamma \vdash y : \SID}  \hspace{10ex}
\inferrule*[right=($D_{8}$)]{\inferrule {\Gamma \vdash x_1 : \SID,~\Gamma \vdash x_2 : \SID,~\Gamma \vdash S_1, S_2 : \mathsf{Set}~\mathsf{v}~ \\\\ \LCOP \text{(} y, x_1 \text{)} \wedge \RCOP( y, x_2) \wedge \\\\  supp (x_1, S_1) \wedge supp (x_2, S_2) \wedge S_1 \cap S_2 \text{=} \emptyset}{} }{\Gamma \vdash y : \SID} 
}
\end{mathpar}
\begin{mathpar}
{\footnotesize
\inferrule*[right=($D_{9}$)]{\inferrule {\Gamma \vdash x_1 : \SID,~\Gamma \vdash x_2 : \SID,~\Gamma \vdash S_1: \mathsf{Set}~\RUD,~\Gamma \vdash S_2: \mathsf{Set}~\mathsf{v},\\\\ \ANDOP(y) \wedge  \LCOP ( y, x_1) \wedge \RCOP (y, x_2) \wedge   dom(x_1, S_1) \wedge supp(x_2, S_2)\wedge S_1 \cap S_2 \neq \emptyset}{} }{\Gamma \vdash y : \SID}
}
\end{mathpar}
\begin{mathpar}
{\footnotesize
\inferrule*[right=($D_{a}$)]{\inferrule {\Gamma \vdash x_1 : \SID,~\Gamma \vdash x_2 : \SID,~\Gamma \vdash S_1 : \mathsf{Set}~\RUD,~ \\\\~\Gamma \vdash S_2: \mathsf{Set}~\mathsf{v},~ \OROP(y) \wedge \LCOP \text{(} y, x_1 \text{)} \wedge \RCOP ( y, x_2) \wedge \\\\  dom (x_1, S_1) \wedge supp (x_2, S_2) \wedge S_1 / S_2 \neq \emptyset}{} }{\Gamma \vdash y : \SID}
\hspace{10ex}
\inferrule*[right=($D_{b}$)]{\inferrule {\Gamma \vdash x_1 : \RUD,~\Gamma \vdash x_2 : \RUD,~\Gamma \vdash S_1 : \mathsf{Set}~\RUD,~ \\\\ ~\Gamma \vdash S_2 : \mathsf{Set}~\mathsf{v},~\ANDOP \text{(} y \text{)} \wedge \LCOP \text{(} y, x_1 \text{)} \wedge \RCOP\text{(} y, x_2\text{)} \wedge \\\\  dom \text{(}x_1, S_1 \text{)} \wedge supp \text{(}x_2, S_2 \text{)} \wedge S_2 / S_1 \neq \emptyset}{} }{\Gamma \vdash y : \SID}
}
\end{mathpar}
\begin{mathpar}
{\footnotesize
\inferrule*[right=($D_{c}$)]{\inferrule {\Gamma \vdash x_1 : \RUD,~\Gamma \vdash x_2 : \RUD,~\Gamma \vdash S_1: \mathsf{Set}~\RUD,~\Gamma \vdash S_2: \mathsf{Set}~\mathsf{v},  \\\\  ~\OROP \text{(} y \text{)} \wedge ~\LCOP \text{(} y, x_1 \text{)} \wedge \RCOP\text{(} y, x_2\text{)} \wedge  dom \text{(}x_1, S_1 \text{)} \wedge supp \text{(}x_2, S_2 \text{)} \wedge S_2 / S_1 \neq \emptyset}{} }{\Gamma \vdash y : \SID}  
}
\end{mathpar}
\begin{mathpar}
{\footnotesize
\inferrule*[right=($D_{d}$)]{\Gamma \vdash x : \RUD}{\Gamma \vdash x : \texttt{NOUKD}} \hspace{1em} \hspace{5ex}
\inferrule*[right=($D_{e}$)]{\Gamma \vdash x : \SID}{\Gamma \vdash x : \texttt{NOUKD}} \hspace{1em} \hspace{5ex}
\inferrule*[right=($D_{f}$)]{\Gamma \vdash x : v,~\NOTOP \text{(} y \text{)} \wedge \LCOP \text{(}y, x\text{)}}{\Gamma \vdash y : v}
\hspace{5ex}
\inferrule*[right=($D_{10}$)]{\Gamma \vdash x : \mathsf{bool},~ x \text{=} \mathsf{true}}{\Gamma \vdash x : \SID}
}
\end{mathpar}
\begin{mathpar}
{\footnotesize
\inferrule*[right=($D_{11}$)]{\Gamma \vdash x : \mathsf{bool},~ x \text{=} \mathsf{false}}{\Gamma \vdash x : \SID} \hspace{10ex}
\inferrule*[right=($D_{12}$)]{{\inferrule{\Gamma \vdash x : \mathsf{v},~ \Gamma \vdash S_k : \mathsf{Set}~\INKEYOP, \Gamma \vdash S : \mathsf{Set}~\mathsf{v},~ supp\text{(}x, S_{s}\text{)} \wedge S_{s} \cap S_k \text{=} \emptyset}{} }
}{\Gamma \vdash x :  \texttt{NOUKD}} \vspace{1em}
}
\end{mathpar}
\begin{mathpar}
{\footnotesize
\inferrule*[right=($D_{13}$)]{\inferrule {\Gamma \vdash x_1 : \RUD,~\Gamma \vdash x_2 : \RUD,~\Gamma \vdash S_1, S_2 : \mathsf{Set}~\RUD,~ \\\\ 
\LCOP \text{(} y, x_1 \text{)} \wedge \RCOP\text{(} y, x_2\text{)} \wedge \MULOP(y) \wedge
\\\\
\text{(} y \text{)} \wedge dom \text{(}x_1, S_1 \text{)} \wedge dom \text{(}x_2, S_2 \text{)} \wedge S_2 / S_1 \neq \emptyset}{} }{\Gamma \vdash y : \SID}  
%\inferrule*[right=($D_{11}$)]{\Gamma \vdash x_1 : \mathbb{RUD},~\Gamma \vdash x_2 : \mathbb{RUD},~~\Gamma \vdash S_1, S_2 : \mathsf{Set}~\mathsf{v},~
%\mathbb{MUL}\text{(} y\text{)} \wedge dom \text{(}x_1, S_1 \text{)}  \wedge dom \text{(}x_2, S_2 \text{)} 
%\wedge S_1/S_2 \neq \emptyset \wedge \mathbb{LC} \text{(} y, x_1 \text{)} \wedge \mathbb{RC}\text{(} y, x_2\text{)}
%} {\Gamma \vdash y : \mathbb{SID}}
\hspace{10ex}
\inferrule*[right=($D_{14}$)]{\Gamma \vdash x_1 : \RUD,~\Gamma \vdash x_2 : \SID,~\Gamma \vdash S_1 : \mathsf{Set}~\RUD\\\\ \Gamma \vdash~S_2 : \mathsf{Set}~\mathsf{v},~ 
\LCOP \text{(} y, x_1 \text{)} \wedge \RCOP\text{(} y, x_2\text{)}~ \MULOP \text{(} y \text{)} \wedge
\\\\
dom \text{(}x_1, S_1 \text{)} \wedge supp \text{(}x_2, S_2 \text{)} \wedge S_1 / S_2 \neq \emptyset}{\Gamma \vdash y : \SID}
\hspace{1em}
}
\end{mathpar}
\begin{mathpar}
{\footnotesize
\inferrule*[right=($D_{15}$)]{\Gamma \vdash x_1 : \SID,~\Gamma \vdash x_2 : \RUD,~\Gamma \vdash S_1 : \mathsf{Set}~\RUD,~S_2 : \mathsf{Set}~\mathsf{v},~ \\\\ \LCOP \text{(} y, x_1 \text{)} \wedge \RCOP\text{(} y, x_2\text{)} \wedge \MULOP \text{(} y \text{)} \wedge dom \text{(}x_1, S_1 \text{)} \wedge supp \text{(}x_2, S_2 \text{)} \wedge S_2 / S_1 \neq \emptyset}{\Gamma \vdash y : \SID}
}
\end{mathpar}
}
\vspace{-1.5em}
\caption{Proof rules for distribution types, gathered from prior
works~\cite{zhang2018sc,eldib2014synthesis,barthe2015verified}. 
Here, $v$ denotes the type of variable $x$,and is of the following types: $\UKD$, $\SID$ and $\RUD$.
$\texttt{NOUKD}$ denotes the secure type (either $\RUD$ 
or $\SID$). All the predefined relations in $KB$ are the same as in $\alpha$.
}
\label{fig:kbRule}
\vspace{-1em}
\end{figure*}

==> kb_proposition.tex <==
\begin{figure*}
{\footnotesize
\begin{mathpar}
\inferrule*[right=($B_1$)] {b \vee \neg b \equiv true}{} \and
\inferrule*[right=($B_2$)] {b \wedge \neg b \equiv false}{} \and
\inferrule*[right=($B_3$)] {\neg\neg b \equiv b}{} \and
\inferrule*[right=($B_{4}$)] {\neg a \vee \neg b \equiv \neg(a \wedge b)}{}
\end{mathpar}
\begin{mathpar}
\inferrule*[right=($B_{5}$)] {\neg a \wedge \neg b \equiv \neg (a \vee b )}{} \and
\inferrule*[right=($B_6$)]{b \vee false \equiv b}{} \and
\inferrule*[right=($B_7$)]{b \vee true \equiv true}{} \and
\inferrule*[right=($B_8$)]{b \wedge true \equiv b}{} 
\end{mathpar}
\begin{mathpar}
\inferrule*[right=($B_9$)]{b \wedge b \equiv b}{}   \and
\inferrule*[right=($B_a$)]{b \wedge false \equiv false}{} \and
\inferrule*[right=($B_b$)]{b \vee b \equiv b}{}  \and
\inferrule*[right=($B_c$)]{a \wedge (a \vee b) \equiv a}{} 
\end{mathpar}
\begin{mathpar}
\inferrule*[right=($B_d$)]{a \vee(a \wedge b) \equiv a}{} \and
\inferrule*[right=($B_e$)]{a \oplus b \equiv (a \wedge \neg b) \vee ( \neg a \wedge b )}{} \and
\inferrule*[right=($B_f$)]{(a \vee b) \vee c \equiv a \vee c \vee b}{} 
\end{mathpar}
\begin{mathpar}
\inferrule*[right=($B_{10}$)]{(a \wedge b) \wedge c \equiv a \wedge c \wedge b}{} \and 
\inferrule*[right=($B_{11}$)]{a \vee (b \vee c) \equiv a \vee b \vee c}{} \and
\inferrule*[right=($B_{12}$)]{a \wedge (b \wedge c) \equiv a \wedge b \wedge c}{}
\end{mathpar}
}
\vspace{-1.5em}
\caption{Proof rules for propositional logic, to simplify the logic formula and deduce Boolean constants ($true$ and $false$).}
\vspace{-1em}
\label{boolean}
\end{figure*}

==> learner-dtl.tex <==
\subsection{The Decision Tree Learning Algorithm}
\label{sub:learner:dtl}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 1. Features

%\paragraph{Choice of pre-defined features}

Recall that our pre-defined features
(Fig.~\ref{sfig:motivation:synthesis:features:predefined}) include
properties of the AST node, such as $\OPOP(x)$, and properties
referring its left and right children, such as $\OPOP(L) \land
\LCOP(x, L)$. The choice requires some care: having very few features
will cause the learning algorithm to fail, while having too many
features will increase the risk of overfitting. Our synergistic
combination of DTL with SyGuS-based on-demand feature synthesis can be
seen as a compromise between these extremes.

% \begin{figure}
% % Analyzer & ::= \lambda x. stmt \\
% % stmt     & ::= \begin{aligned}[t]
% %                  & switch(F)
% %                    case1 => stmt;
% %                    ...
% %                    case|F| => stmt \\
% %                  & \mid \TYPE(x)
% %                \end{aligned}
% \[
% \begin{array}{rrcl}
%   \text{Feature} & \mathcal{F} & \Coloneqq & F? \mid \OPOP(x) \mid \IN(x) \\
%                  &             & \mid      & \OPOP(L) \land \LCOP(x, L) \mid \OPOP(R) \land \RCOP(x, R) \\
%                  &             & \mid      & \TYPE(L) \land \LCOP(x, L) \mid \TYPE(R) \land \RCOP(x, R) \\
%   %
%                  & \OPOP       & \Coloneqq & \ANDOP \mid \OROP \mid \NOTOP \mid \XOROP \mid \MULOP \mid \LEAFOP \\
%   %
%                  & \IN         & \Coloneqq & \INRANDOP \mid \INKEYOP \mid \INPUBOP \\
%   %
%                  & \TYPE       & \Coloneqq & \UKD \mid \SID \mid \RUD
% \end{array}
% \]
% \caption{Syntax $\mathcal{L}_{D}$ of features used in DTL.}
% %F? represents the feature synthesized from $FeatureSyn$().}
% \label{fig:learner:dtl:predefined}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 2. Entropy-Guided Decision Tree Learning

%\paragraph{Entropy-guided decision tree learning}

$\DTL(\mathcal{E}, \mathcal{F})$ is an \emph{entropy-guided} greedy learner~\cite{rokach2005top}.
The entropy of a set is a measure of the diversity of its labels:

{\footnotesize
\vspace{-1em}
$$
\begin{array}{l}
  H(\mathcal{E})  = -\sum_{t \in \TYPE} \Pr(\TYPE(x) = t) ~ \log(\Pr(\TYPE(x) = t)) \\\\
  H(\mathcal{E} \mid f)  = \sum_{i \in \Range(f)} H(\mathcal{E} \mid f(x) = i)
\end{array}
$$
}%

\noindent
%
%Thus, the feature $f = f^*$ that minimizes the conditional entropy $H(\mathcal{E} \mid f)$ (lines~7--12 in Algorithm~\ref{alg:learner} is greedily chosen, to partition the training set $\mathcal{E}$ before processing each subset in $\DTL(\mathcal{E} \rvert_{f^*(x) = i},\mathcal{F} \setminus \{ f^* \})$.
Algorithm~\ref{alg:learner} thus divides the set of training examples
$\mathcal{E}$ using the feature $f = f^*$ that minimizes the conditional entropy $H(\mathcal{E} \mid f)$ (lines~7--12), and recursively invokes the learning algorithm on each subset, $\DTL(\mathcal{E} \rvert_{f^*(x) = i},\mathcal{F} \setminus \{ f^* \})$.

Observe that $H(\mathcal{E}) = 0$ if $\Pr(\TYPE(x)=t)=100\%$, meaning
\emph{purity} or all examples $x \in \mathcal{E}$ share the same type
$\TYPE(x) = t$. The difference between $H(\mathcal{E})$ and
$H(\mathcal{E} \mid f)$ is also referred to as the \emph{information
  gain}. If the learner cannot find a feature with strictly positive
information gain (line~4), it will invoke the feature synthesis
algorithm on line~5.



==> learner-sygus.tex <==
\subsection{The On-Demand Feature Synthesis Algorithm}
\label{sub:learner:sygus}

\begin{algorithm}[t]
{\footnotesize
\input{images/learner/feature-syn.tex}
}
\caption{$\FeatureSyn$($\mathcal{E}$).}
\label{alg:learner:sygus}
\end{algorithm}

\setlength{\textfloatsep}{10pt plus 1.0pt minus 2.0pt}
\begin{figure}
{\footnotesize
  \[
    R_f = \left\{
            \begin{array}{rcl}
              f(x) & \gets & p_{in}(x), \\
              f(x) & \gets & q_{in}(x, y), \\
              f(x) & \gets & p_{in}(x, y) \land q_{in}(x, y), \\
              f(x) & \gets & q_{in}(x, y) \land f(y), \\
              f(x) & \gets & q_{in}(x, y) \land p_{in}(x) \land f(y)
            \end{array}
          \right\}
  \]

  \[
    R_g = \left\{
            \begin{array}{rcl}
              g(x, y) & \gets & q_{in}(x, y), \\
              g(x, y) & \gets & p_{in}(x) \land q_{in}(x, y), \\
              g(x, y) & \gets & q_{in}(x, z) \land g(z, y), \\
              g(x, y) & \gets & q_{in}(x, z) \land p_{in}(x) \land g(z, y)
            \end{array}
          \right\}
  \]

\[
  R_h = \left\{
          \begin{array}{rcl}
            h(x) & \gets & f(x) \land p_{in}(x) \land q_{in}(x, y), \\
            h(x) & \gets & g(x, y) \land p_{in}(x) \land q_{in}(x, y), \\
            h(x) & \gets & f(x) \land g(x, y) \land p_{in}(x) \land q_{in}(x, y)
          \end{array}
        \right\}
\]

\[
  \begin{array}{rcl}
    p_{in}(x)    & \Coloneqq & \ANDOP(x) \mid \OROP(x) \mid \NOTOP(x) \mid \XOROP(x) \mid \MULOP(x) \mid \LEAFOP(x) \\
                 & \mid      & \INRANDOP(x) \mid \INKEYOP(x) \mid \INPUBOP(x) \\
                 & \mid      & p_{in} \land p_{in} \mid p_{in} \lor p_{in} \mid \lnot p_{in} \\
    q_{in}(x, y) & \Coloneqq & \LCOP(x, y) \mid \RCOP(x, y) \mid x = y \\
                 & \mid      & q_{in}(x, y) \land q_{in}(x, y) \mid q_{in}(x, y) \lor q_{in}(x, y) \\
                 & \mid      & \lnot q_{in}(x, y)
  \end{array}
\]
}%\footnotesize

\caption{Syntax of the DSL for synthesizing new features.}
\label{fig:learner:sygus:metarules}
\end{figure}

%\ignore{%% chao: removed the background on Datalog
\emph{Representing new features.}
%
We represent the newly synthesized features as Datalog programs. Datalog is an increasingly popular medium to express
complex static analyses~\cite{Reps1995, bddbddb, jordan2016souffle, doop}, and its recursive nature enables the newly
learned features to represent arbitrarily deep properties of AST nodes.
%
%Briefly, a Datalog program is a collection of rules, 
%examples of which we saw in Figure~\ref{fig:motivation:setting:rules}. 
A Datalog rule is a constraint of the form
\begin{alignat}{1}
  h(\bm{x}) & \gets b_1(\bm{y}_1) \land b_2(\bm{y}_2) \land \dots \land b_n(\bm{y}_n), \label{eq:learner:sygus:rule}
\end{alignat}
where $h$,$b_1$\dots$b_n$ are relations with pre-specified arities and schemas, and where $\bm{x}$,
$\bm{y}_1$\dots$\bm{y}_n$ are vectors of typed variables. Each rule  %is a universally quantified formula in first order logic, which
can be interpreted as a logical implication: if
$b_1$\dots$b_n$ are true, then so is $h$.
The semantics of a Datalog program is defined as the \emph{least-fixed point} of rule application~\cite{Alice}: the solver starts with
empty output relations, and repeatedly derives new output tuples until no new tuples can be derived.
%
%}%% chao: removed the background on Datalog


%\paragraph{Syntax-guidance using meta-rules}

%Program synthesis and machine learning algorithms commonly restrict
%the space of target concepts and bias the search to speed up
%computation and improve generalization. One particularly influential
%form of bias has been to constrain the syntax of target concepts: this
%has been formalized as the SyGuS problem~\cite{alur2013syntax} and as
%meta-rules in inductive logic programming~\cite{Muggleton:MIL,
%  si2018syntax}.
%

\input{kb_proposition}

Program synthesis commonly restricts the space of 
target concepts and biases the search to speed up
computation and improve generalization. One form of 
bias has been to constrain the syntax: 
this has been formalized as the 
SyGuS problem~\cite{alur2013syntax} and as
meta-rules in inductive logic programming~\cite{Muggleton:MIL,
si2018syntax}. A meta-rule is construct of this form
%We assume features are defined by meta-rules of the form below to reduce the search space:
% 
\begin{alignat}{1}
  X_h(\bm{x}) & \gets X_1(\bm{y}_1) \land X_2(\bm{y}_2) \land \dots \land X_n(\bm{y}_n) \label{eq:learner:sygus:metarule}
\end{alignat}
Here, $X_h$, $X_1$, $X_2$, \dots, $X_n$ are \emph{relation variables} whose instantiation yields a concrete rule. 
Fig.~\ref{fig:learner:sygus:metarules} shows the meta-rules
used in our work. 
For example, instantiating the meta-rule $f(x) \gets
q_{in}(x, y) \land p_{in}(x) \land f(y)$ with $q_{in}(x, y) = \RCOP(x,
y)$ and $p_{in}(x) = \XOROP(x)$ yields  $f(x) \gets
\RCOP(x, y) \land \XOROP(x) \land f(y)$.
%
There are three variations of the final target relation schema,
$f(x)$, $g(x, y)$ and $h(x)$, where $x$ and $y$ denote AST nodes.


We formalize the synthesis problem as that of choosing a relation $R
\in \{ f(x), g(x, y), h(x) \}$ and finding a subset $P_D$ of its
instantiated meta-rules from Fig.~\ref{fig:learner:sygus:metarules}
such that the resulting Datalog program $P_D$ has strictly positive information
gain on the provided training examples $\mathcal{E}$.

% TODO: We use f(x) for the relation schema of the new feature, and also for the new feature itself.
% Resolve this overloading.



%%%%
% 2a. UC2RPQ~\cite{calvanese2005decidable, calvanese2003reasoning, barcelo2014does}
% TODO: Talk to Jingbo about UC2RPQ
% TODO: We have already discussed this in Section 2. Please feel free to delete the following paragraph

\ignore{
In the subsequent soundness verification pass, our goal will be to determine if the learned analysis rules, represented as a Datalog program, is valid for all possible (unseen) programs.  While this problem is undecidable for general Datalog programs~\cite{calvanese2005decidable}, it does admit decision
procedures for certain restricted classes of programs, notably the UC2RPQ subset (Union of Conjunctive 2-Way Regular
Path Queries; see~\cite{calvanese2005decidable, calvanese2003reasoning, barcelo2014does}). We therefore carefully choose
the meta-rules in Figure~\ref{fig:learner:sygus:metarules} to only produce concrete programs from the UC2RPQ fragment.
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 3. (Semantic Specification and) Synthesis Algorithm

% TODO: Do we want to keep this part? The algorithm is kind of obvious.

%\paragraph{The feature synthesis algorithm}

%%%% Explanation of Alg 2
%   1. apply the input relations to the example set and obtain the facts
%   2. choose the head of the rule (intensional predicate) in the meta rule (f,g,h)
%       Say I choose h
%   3. construct the possible derivation paths to the h(x), so here it has 2^3 templates
%      Say I choose template 1 and template 3
%   4. for each path (consisting template 1 and template 3)
%       we start from template 1
%   5. we are gonna select the set for each predicate shown in the body of the template 1
%   We say there are #n  options for defining f(x), and for P_In(x), 2^9 possible instiations, and for
%   q_in(x,y), 2^3 instantiations. so basically for n*2^9*2^3
%       we start from rule 3
%       followed by the above approach, assuming there are #m options for defining g(x,y), there are 
%       m*n*2^9*2^3

% if (h(E) - h(E | P_D) > 0) {
%    ...
% }

Algorithm~\ref{alg:learner:sygus} shows the procedure, which
repeatedly instantiates the meta-rules from
Figure~\ref{fig:learner:sygus:metarules} and computes their
information gain. It successfully terminates when it discovers a
feature that can improve classification. Otherwise, it
returns failure (upon timeout) and invokes
$\DTL(\mathcal{E}, \mathcal{F})$ to conservatively classify
the decision tree node as being of type $\UKD$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 4. Three Examples

% 4a. Feature with zero information gain (TODO!)
% 4b. Feature with negative information gain, used in sound rule
% 4c. Feature with positive information gain, used in unsound rule

\begin{example}
\label{ex:learner:sygus}
Given $\mathcal{E} = \{ (\mathlst{b4}, \RUD), (\mathlst{n1}, \UKD) \}$
shown in Fig.~\ref{sfig:motivation:example:program}, the synthesizer
may alternatively learn the rules in
Equations~\ref{eq:learner:sygus:zeroGain},
\ref{eq:learner:sygus:valid} and~\ref{eq:learner:sygus:invalid}.

\vspace{-1em}
{\footnotesize
\begin{alignat}{2}
% save some space
%\setlength{\jot}{1pt}
%
  f(x) & \gets \INRANDOP(x), \label{eq:learner:sygus:zeroGain} \\
  f(y) & \gets \LCOP(y, x) \land f(x), \nonumber \\
  f(y) & \gets \RCOP(y, x) \land f(x), \nonumber \\ %\\ &  \nonumber 
  \RUD(x) & \gets \XOROP(x) \land \LCOP(x, L) \land \RCOP(x, R) \land \RUD(L) \land f(R). \nonumber
  \\[0.75em]
  g(x, x) & \gets \INRANDOP(x), \label{eq:learner:sygus:valid} \\
  g(y, z) & \gets \LCOP(y, x) \land g(x, z), \nonumber \\
  g(y, z) & \gets \RCOP(y, x) \land g(x, z), \nonumber \\
  h(x) & \gets \LCOP(x, L) \land \RCOP(x, R) \land g(L, x_L) \land g(R, x_R) \land x_L = x_R, \nonumber \\
  \RUD(x) & \gets \XOROP(x) \land \RUD(L) \land \RUD(R) \land \LCOP(x, L) \land \RCOP(x, R) \land \lnot h(x). \nonumber
  %\\&  \nonumber 
  \\[0.75em]
  g(x, x) & \gets \INKEYOP(x), \label{eq:learner:sygus:invalid} \\
  g(y, z) & \gets \LCOP(y, x) \land g(x, z), \nonumber \\
  g(y, z) & \gets \RCOP(y, x) \land g(x, z). \nonumber \\
  h(x) & \gets \LCOP(x, L) \land \RCOP(x, R) \land g(L, x_L) \land g(R, x_R) \land x_L = x_R,  \nonumber \\
  \RUD(x) & \gets \XOROP(x) \land \RUD(L) \land \RUD(R) \land \lnot h(x). \nonumber
\end{alignat} \vspace{-1.5em}
}

Since the information gain of Rule~\ref{eq:learner:sygus:zeroGain}
applying to \{$\mathlst{b4}, \mathlst{n1}$\} is zero, it gets
discarded (Line 6 in Algorithm~\ref{alg:learner:sygus}).  In contrast,
the information gains of Rules~\ref{eq:learner:sygus:valid} and
\ref{eq:learner:sygus:invalid} are both positive.
Rule~\ref{eq:learner:sygus:valid} intuitively requires that both the
left and right operands of $x$ are of type $\RUD$, and that they do
not share any random inputs in computing $\lnot
h(x)$. Rule~\ref{eq:learner:sygus:invalid} requires that the same
secret key be used in the computation of both operands. 
%
While Rule~\ref{eq:learner:sygus:valid} is sound when applied to arbitrary
programs, Rule~\ref{eq:learner:sygus:invalid} is unsound. 
In
the next section, we will present an algorithm that can check the
soundness of these learned rules. 
\end{example}



==> learner.tex <==
\section{Learning the Type-inference Rules} % TODO: or, Learning Inference Rules, or Analysis Rule Induction
\label{sec:learner}

%As discussed in Section~\ref{sec:motivation}, \GPS{} consists of an
%interaction loop between the analysis rule learner and the soundness
%verifier. 
We formally describe the analysis rule learner 
in Algorithm~\ref{alg:learner}. The input
consists of a set of labeled examples, $\mathcal{E}$,
%$ = \{ (x_1, \TYPE(x_1)), (x_2, \TYPE(x_2)), \dots, (x_n, \TYPE(x_n)) \}$, 
and a
set of pre-defined features, $\mathcal{F}$,
%$ = \{ f_1, f_2, \dots, f_k \}$. 
and the output $\mathcal{T}$ is a set of type-inference rules
consistent with training examples.
%
Each training example $(x, \TYPE(x)) \in \mathcal{E}$ consists of an
AST node $x$ in a program and its distribution type $\TYPE(x)$.



At the top level, the learner uses the standard \emph{decision tree
  learning (DTL)} algorithm~\cite{rokach2005top} as the baseline.
However, if it finds that the current set $\mathcal{F}$ of
classification features is insufficient, it invokes a
\emph{syntax-guided synthesis (SyGuS)} algorithm to synthesize a new
feature $f$ with strictly positive information gain to augment
$\mathcal{F}$.  This allows the learner to combine the efficiency of
techniques that learn decision trees with the expressiveness of syntax
guided synthesis; similar ideas have been fruitfully used in other
applications of program synthesis, see for
example~\cite{alur2017scaling}.




While the top-level classifier (e.g.,
Fig.~\ref{sfig:motivation:example:tree4},
\ref{sfig:motivation:synthesis:features:tree1},
\ref{sfig:motivation:synthesis:features:tree2} and
\ref{fig:motivation:proof:tree3}) has a bounded number of decision
points, the synthesized features (e.g.,
Fig.~\ref{sfig:motivation:setting:rules:learned}) may be
recursive. Furthermore, the newly synthesized features $f$ are
inducted as first-class citizens of $\mathcal{F}$, and can
subsequently be used at any level of the decision tree (see, for
example Fig.~\ref{sfig:motivation:example:tree4}
and~\ref{fig:motivation:proof:tree3}).
%
Next, we present the DTL and SyGuS subroutines respectively.



\begin{algorithm}[t]
\caption{$\DTL(\mathcal{E}, \mathcal{F})$ --- Decision Tree Learning.}
\label{alg:learner}
{\footnotesize
\input{images/learner/dtl.tex}
}
\end{algorithm}



% \clearpage
\input{learner-dtl.tex} % \clearpage
\input{learner-sygus.tex}


==> motivation-architecture.tex <==
%\subsection{Overall Architecture of the \GPS{} System}
%\label{sub:motivation:architecture}

To summarize, the \emph{learner} repeatedly applies decision tree
learning and synthesizes new features to learn candidate analyses that
correctly classify all training examples and are consistent with all
previously discovered abstract counter-examples, as shown in
Fig.~\ref{overview}. 
%
The \emph{prover} determines whether the learned analysis rules are
sound.  Each subsequent counter-example is fed back to the rule
learning algorithm which restarts the learning process on the
augmented dataset, until either all synthesized rules are sound or a
time bound is exhausted.
%
%For the AES benchmark~\cite{coron2013higher}, our learned analyzer is
%more than two orders of magnitudes faster than the human-written
%baseline~\cite{wang2019mitigating} without sacrificing either
%soundness or empirical accuracy. Moreover, under some benchmarks such
%as Messerges Boolean function~\cite{bayrak2013sleuth}, the learned
%analyzer is even more accurate than the manually written analyzer
%because it performs more sophisticated constant propagation. 
In the next three sections, we first describe the technical backgound,
and then present the learner and the prover respectively.
%
%We will then present our experimental results in
%Section~\ref{sec:experiment}, and conclude with a short survey of
%related work.


==> motivation-proof.tex <==
\subsection{Proving Soundness of Learned Analysis Rules}
\label{sub:motivation:proof}

While the learned analysis rules are \emph{correct by construction}
for the training examples, they may still be unsound when applied to
unseen programs. We observe this, for example, in the leaves
highlighted in red in
Fig.~\ref{sfig:motivation:synthesis:features:tree2}. 
%
Thus, \GPS{} tries to confirm their soundness against the
domain-specific knowledge base $KB$. 
%We assume that $KB$ is specified
%as a set of first-order inference rules, such as those shown in
%Fig.s~\ref{boolean} and~\ref{fig:kbRule}. 
In the context of our running example---confirming soundness means
proving that every variable $x$ that is assigned type $\RUD(x)$
(resp. $\SID(x)$) by the learned analysis rule $\alpha$ is also
certified $\RUD(x)$ (resp. $\SID(x)$) by $KB$.


We formalize the soundness proof as a Datalog query containment
problem,
%
%Because the query containment problem for general Datalog programs is
%famously undecidable~\cite{calvanese1998decidability}, we restrict the
%meta-rules used by the feature synthesis algorithm in
%Section~\ref{sub:motivation:synthesis} to only generate analysis rules
%within the restricted UC2RPQ class of queries~(Union of Conjunctive
%2-way Regular Path Queries), for which query containment is known to
%be decidable~\cite{calvanese2003reasoning, calvanese2005decidable,
%  barcelo2014does}.
%
and propose an algorithm based on bounded unrolling and
$k$-induction to check it. 



% TODO: Why does the soundness check produce abstract counter-examples rather than concrete counter-examples?

% TODO: "prohibits" vs "disincentivizes"

When applied to the candidate analysis of
Fig.~\ref{sfig:motivation:synthesis:features:tree2}, the check results
in the five counter-examples $CE_1, \dots, CE_5$ with distribution type $\UKD(CE_i)$
shown in Fig.~\ref{sfig:motivation:proof:cex}.  Each
counter-example indicates the unsoundness of one path from the root of
the decision tree to a classification node. These counter-examples
contain \emph{missing features} and consequently do not define
concrete ASTs. Thus, each of these \emph{abstract} counter-examples is
a set of feature valuations $\pi = \{ f_1 \mapsto v_1, f_2 \mapsto
v_2, \dots, f_k \mapsto v_k \}$ that the current candidate analysis
misclassifies, and feeding them back to the learner prohibits
subsequent candidate analyses from classifying variables that satisfy
$\pi$.

With these new constraints from abstract counter-examples, the learner
learns the new candidate analysis shown in
Fig.~\ref{fig:motivation:proof:tree3}. This new candidate analysis
still has four unsound candidate rules, which results in additional
abstract counter-examples when it is subjected to the soundness
check. We repeat this back-and-forth between the rule learner and the
soundness prover: after 11 iterations and after processing 27
counter-examples in all, \GPS{} learns the rules initially presented
in Fig.~\ref{sfig:motivation:example:tree4}, all of which have been
certified to be sound.

\subsection{Overall Architecture of the \GPS{} System}
%\emph{Summarize the architecture of \GPS{}.} 
We summarize the architecture of \GPS{} in Fig.~\ref{overview}.
The learner repeatedly applies DTL and SyGuS to learn candidate analyses that correctly classify training samples and are consistent with newly-added abstract counter-examples. Next, prover checks the soundness of the learned analysis. Each subsequent counter-example is fed back to the learner which restarts the rule learning process on augmented dataset, untill either all synthesized rules are sound or a time bound is exhausted.

%\begin{figure*}
%\centering
%\input{images/motivation/tree3.tex}
%\caption{Candidate analysis learned after one round of feedback from
%  the soundness verifier. The leaves shown in green and red correspond
%  to sound and unsound analysis rules respectively.}
%\label{fig:motivation:proof:tree3}
%\end{figure*}


==> motivation-setting.tex <==
\subsection{Problem Setting}
\label{sub:motivation:setting}
Given such masked programs, users want to determine if they succeed in
eliminating side-channel vulnerabilities: in particular, if each
intermediate result is uniformly distributed ($\RUD$) or at least independent
of the sensitive inputs ($\SID$). The desired static analysis thus associates each
variable $x$ (e.g., $n_1$) with the elements of a
three-level abstract domain, $\RUD$, $\SID$ or $\UKD$, indicating that
$x$ is uniformly distributed ($\RUD$), secret independent 
($\SID$), or unknown ($\UKD$) and therefore
potentially vulnerable.  

  %
  \textcolor{red}{
  The decision tree in Fig.~\ref{sfig:motivation:example:tree4}
  represents the desired static analyzer, which accurately classifies most
  variables of the training corpus, and is also sound when applied
  to new programs. Given variable $x$, the decision tree
  leverages the features of $x$---such as the operator 
  type of $x$ ($\OPOP$(x) := $\ANDOROP$(x)$|\XOROP$(x))
  and the types of $x$'s operands (e.g. $\TYPE$(L), $\TYPE$(R))---and maps 
  $x$ to its corresponding distribution type.
   The white nodes of Fig.~\ref{sfig:motivation:example:tree4}
  represent pre-defined features, while the grey nodes represent output classes
  (associated types).
  Each path from the root to leaf node corresponds to one
  analysis rule.
  The complete set of pre-defined features are
  demonstrated in Fig.~\ref{sfig:motivation:synthesis:features:predefined}.
  }
  
  
 Designing such side-channel analyses has been the focus of intense
research, see for example~\cite{wang2019mitigating, zhang2018sc,
  barthe2018maskverif, wang2017security, barthe2016strong,
  barthe2015verified,chen2017precise,tizpaz2019quantitative}.
Unfortunately, it requires expert knowledge in both computer security
and program analysis, and invariably involves delicate trade-offs
between accuracy and scalability. Our goal in this work is to assist
the analysis designer in automating the development.  This problem has
also been the subject of exciting research~\cite{david2015using,
  bielik2017learning}; however, these approaches typically either
require computationally intensive deductive synthesis or cannot 
%from fragments of second-order logic 
guarantee soundness 
%of the learned
%analyzers 
and thus produce errors in both directions, including false
alarms and missed bugs.

In contrast, \GPS{} combines inductive synthesis from user annotations
with logical entailment checking against a more comprehensive, known-to-be-correct set of
proof rules that form the knowledge base ($KB$). It takes as input
training programs like the one in
Fig.~\ref{sfig:motivation:example:program}, where the labels
correspond to the types of program variables ($\RUD$/$\SID$/$\UKD$ for intermediate results and
$\INRANDOP$/$\INPUBOP$/$\INKEYOP$ for inputs). The users are free to
annotate as many or as few of these types as they wish: this affects
only the precision of the learned analyzer and not its soundness.
Second, \GPS{} also takes as input the knowledge base $KB$, consisting of
proof rules that describe axioms of propositional logic
(Fig.~\ref{boolean}) and properties of the distribution types
(Fig.~\ref{fig:kbRule}). In return, \GPS{} produces as output
a set of Datalog rules which simultaneously achieves high accuracy
on the training data and provably sound with respect to $KB$.

The proof rules for $KB$ %distribution types of, in particular, 
were collected from published papers on masking
countermeasures~\cite{zhang2018sc, wang2019mitigating,
barthe2015verified}.  We emphasize that $KB$ is not necessarily an
executable static analyzer since repeated application of these proof
rules need not necessarily reach a fixpoint and terminate in finite
time; 
%instead, they are merely used to prove the soundness of our learned analysis rules.
Furthermore, even in cases
where it does terminate, $KB$ may be computationally expensive and
infeasible for application to large programs.
As a concrete example, we compare excerpts of the rules learned by
\GPS{} in Fig.~\ref{sfig:motivation:setting:rules:learned} 
to the corresponding rules from SCInfer~\cite{zhang2018sc}---a 
sophisticated human-written analysis---in Fig.~%
\ref{sfig:motivation:setting:rules:scinfer}.
\textcolor{red}{
$\LCOP(x,L)$ and $\RCOP(x, R)$ arises in both versions, 
indicating that the variable $L$ and $R$ are the left and right
operands of $x$ respectively.
Specifically, in Fig.~\ref{sfig:motivation:setting:rules:scinfer}, $\SUPPOP(x, y)$
indicates that $y$ is used in the computation of $x$ syntactically while $ \DOMOP(x, y)$
denotes that random variable $y$ is used in the computation of $x$ semantically.
} 
Observe the computationally
expensive set-theoretic operations in the
human-written version to the simpler rules learned by \GPS{} without
loss of soundness or perceptible loss in accuracy. These points are
also borne out in our experiments in Table~\ref{tbl:FSE19}, where
SCInfer takes $>$45 minutes on some Keccak benchmarks, while our
learned analysis takes $<$5 seconds.

\GPS{} consists of two phases: First, it learns a set of
type-inference rules---alternatively represented either as Datalog
programs or as decision trees---that are consistent with the training
data. Second, it proves these rules against the knowledge base.  
%
%Counter-examples of the failed proofs are passed back to prevent these
%rules from being learned again.  
In the next two subsections, we will explain the rule learning and
soundness proving processes respectively.


==> motivation-synthesis.tex <==
\subsection{Feature Synthesis and Rule Learning}
\label{sub:motivation:synthesis}

% TODO: Give example of grammar of meta-rules. Connect to UC2RPQ in Section 2.3.

The learned analyzer associates each node $x$ of a program's abstract
syntax tree (AST) with an element of the distribution type $\{
\UKD(x), \SID(x), \RUD(x) \}$. 
We may therefore interpret the analyzer
as a decision tree that, by considering various features of an AST
node, maps it to a type. With a pre-defined set of features, such as
those shown in
Fig.~\ref{sfig:motivation:synthesis:features:predefined}, analyzers of
this form can be learned with classical decision tree learning (DTL)
algorithms.  Fig.~\ref{sfig:motivation:synthesis:features:tree1} shows
such an analyzer, learned from the labeled program of
Fig.~\ref{sfig:motivation:example:program}.

Unfortunately, the pre-defined features may not be strong enough
to distinguish between nodes with different training labels, e.g.,
\lstinline|b4| and \lstinline|n1| from the training program, which
have distinct labels $\RUD(\mathlst{b4})$ and $\UKD(\mathlst{n1})$,
but after being sifted into the node highlighted in red in
Fig.~\ref{sfig:motivation:synthesis:features:tree1}, cannot be
separated by any of the features from
Fig.~\ref{sfig:motivation:synthesis:features:predefined}. 
%
To ensure soundness, the learner would be forced to conservatively
assign the label $\UKD(x)$, which sacrifices the accuracy. 

% TODO: Confirm _set of inference rules_ vs _inference rule in the sentence:
% ... and the target specification is ...
\GPS{} thus includes a \emph{feature} synthesis engine, triggered whenever
the learner fails to distinguish between two differently labeled
variables. In tandem with recursive feature synthesis,
\GPS{} overcomes the limited expressiveness of DTL by enriching
syntax space to capture more desired patterns.
Observe that paths of a decision tree can
be represented as Datalog rules, e.g., the red path
in
Fig.~\ref{sfig:motivation:synthesis:features:tree1} is equivalent to
%
{%\footnotesize
\[
  \UKD(x) \gets \XOROP(x) \land \XOROP(R) \land \RUD(L) \land \LCOP(x, L) \land \RCOP(x, R).
\]
}%
%
Viewing this in Datalog also allows us to conveniently describe
\emph{recursive} features, and reduce \emph{feature synthesis} to an
instance of syntax-guided synthesis (SyGuS).
%
Syntactically, the analysis rules corresponding to new features
are instances of a pre-defined set of \emph{meta-rules}, and the
target specification is to produce a Datalog program for a relation
$f(x)$ that has strictly positive information gain for the variables
under consideration (see Section~\ref{sec:learner} for details).

% TODO: Are f(x) and g(x, r) two features or just one feature?
In our running example, the synthesizer produces the feature $f(x)$
shown in Fig.~\ref{sfig:motivation:setting:rules:learned}, which
intuitively indicates that some random input $r$ is used to compute
both operands of $x$.
%
With this new feature, the learner can distinguish between
\lstinline|b4| and \lstinline|n1|, and produce the rule shown in
Fig.~\ref{sfig:motivation:synthesis:features:tree2}, which correctly
classifies all variables of the training program. 
%
Observe that the rules defining $f(x)$ in
Fig.~\ref{sfig:motivation:setting:rules:learned} involve a newly
introduced predicate $g(x, r)$ and recursive structure that can
classify variables based on arbitrarily deep properties of the
abstract syntax tree. 
  
\begin{figure}
  \centering
  \scalebox{0.7}{
    \begin{tabular}{lcccccc}
      \toprule
      & \tikz{\node [root2] {$\OPOP(x)$}} & \tikz{\node [root2] {$\OPOP(L)$}} & \tikz{\node [root2] {$\OPOP(R)$}}
      & \tikz{\node [root2] {$\TYPE(L)$}} & \tikz{\node [root2] {$\TYPE(R)$}} & $f(x)$ \\
      \midrule
      $CE_1$ & $\ANDOROP$ & -1 & -1         & -1     & -1 & -1 \\
      $CE_2$ & $\XOROP$   & -1 & $\LEAFOP$  & -1     & -1 & -1 \\
      $CE_3$ & $\XOROP$   & -1 & $\XOROP$   & $\SID$ & -1 & -1 \\
      $CE_4$ & $\XOROP$   & -1 & $\ANDOROP$ & $\RUD$ & -1 & -1 \\
      $CE_5$ & $\XOROP$   & -1 & $\ANDOROP$ & $\SID$ & -1 & -1 \\
      \bottomrule
    \end{tabular}
  }
  %
  %\vspace{-1em}
  \caption{The table denotes
    the abstract counter-examples produced during the soundness
    verification of the candidate analyzer shown in Fig.~\ref{sfig:motivation:synthesis:features:tree2}.
    }
    \label{sfig:motivation:proof:cex}
    \vspace{-1em}
\end{figure}

\setlength{\textfloatsep}{10pt plus 1.0pt minus 2.0pt}
\begin{figure}
  \centering
  %
  \scalebox{0.7}{\input{images/motivation/tree3.tex}}
  \caption{It shows candidate analysis learned after one round of feedback from the soundness verifier. The leaves shown in green and red correspond to sound and unsound analysis rules respectively.}
  \label{fig:motivation:proof:tree3}
  %
  \vspace{-1em}
\end{figure}


%\begin{figure}
%  \centering
  %
%  \begin{subfigure}[m]{0.47\textwidth}
%  \scalebox{0.8}{\input{images/motivation/tree2.tex}}
%  \caption{}
%  \label{sfig:motivation:synthesis:features:tree2}
%  \end{subfigure}
  %
%  \begin{subfigure}[m]{0.47\textwidth}
%  \centering
%  \scalebox{0.8}{
%    \begin{tabular}{lcccccc}
%      \toprule
%      & \tikz{\node [root] {$\OPOP(x)$}} & \tikz{\node [root] {$\OPOP(L)$}} & \tikz{\node [root] {$\OPOP(R)$}}
%      & \tikz{\node [root] {$\TYPE(L)$}} & \tikz{\node [root] {$\TYPE(R)$}} & $f(x)$ \\
%      \midrule
%      $AC_1$ & $\ANDOROP$ & -1 & -1         & -1     & -1 & -1 \\
%      $AC_2$ & $\XOROP$   & -1 & $\LEAFOP$  & -1     & -1 & -1 \\
%      $AC_3$ & $\XOROP$   & -1 & $\XOROP$   & $\SID$ & -1 & -1 \\
%      $AC_4$ & $\XOROP$   & -1 & $\ANDOROP$ & $\RUD$ & -1 & -1 \\
%      $AC_5$ & $\XOROP$   & -1 & $\ANDOROP$ & $\SID$ & -1 & -1 \\
%      \bottomrule
%    \end{tabular}
%  }
%  \caption{}
%  \label{sfig:motivation:proof:cex}
%  \end{subfigure}
%  \caption{Candidate static analyzer produced after one round of
%    feature synthesis
%    (Fig.~\ref{sfig:motivation:synthesis:features:tree2}). The blue
%    paths corresponds to the rule $\RUD(x) \gets \XOROP(x) \land LC(x,
%    L) \land RC(x, R) \land \XOROP(R) \land \RUD(L) \land \lnot
%    f(x)$. Unfortunately, even though this analysis achieves 100\%
%    training accuracy, the leaf nodes highlighted in red correspond to
%    unsound predictions.  Fig.~\ref{sfig:motivation:proof:cex} shows
%    the abstract counter-examples produced during the soundness
%    verification.}
%\end{figure}


==> motivation.tex <==
\section{Motivation}
\label{sec:motivation}

%% move the figure of motivation section to intro to make it in the second page
\begin{figure*} [t!] %[hbt!]
  \centering
  \subfloat[]
  {
  \hspace{-1em}
    \scalebox{0.75}{
      \renewcommand{\arraystretch}{1.3}
      \begin{tabular}{|p{0.1\textwidth}@{}|p{0.35\textwidth}}
        \cline{1-1}
        %{\footnotesize User \allowbreak Labels} & \\
        %
        \begin{minipage}{0.16\textwidth}
          \textcolor{DarkGreen}{
            \lstinputlisting{images/motivation/ua-brief.cbool}
          }
        \end{minipage}
        &
        \begin{minipage}{0.8\textwidth}
          \lstinputlisting{images/motivation/keccak-brief.cbool}
        \end{minipage}
        \\
        \cline{1-1}
      \end{tabular}
    }
    \label{sfig:motivation:example:program}
  }
  %
  %\hspace{5ex} 
  %\hfill
  %
  \subfloat[]
  {
  \adjustbox{raise=-6pc}{
    %\hspace{-1em}
    \scalebox{0.75}{
      \input{images/motivation/tree4.tex}
    }
    \label{sfig:motivation:example:tree4}
    }
  }
  % TODO: Which rules are not sound? Identify them in the caption!
  \caption{The program on the left is a perfectly masked $\chi$
    function from MAC-Keccak.
    %The program takes three secret variables \lstinline|i1|, \lstinline|i2|, \lstinline|i3| as input and computes the function \lstinline|n1 = i1 $\oplus$ ($\lnot$ i2 $\land$ i3)|. This implementation obfuscates its computation using three additional random variables \lstinline|r1|, \lstinline|r2| and \lstinline|r3|.
    %
    The decision tree on the right represents the static analyzer that the user would like to synthesize. Here, $x$ is a program variable, whose
    type is being computed;  $L$ and $R$ are its
    left and right operands, respectively, and $f(x)$ is a synthesized
    feature shown in Fig.~\ref{sfig:motivation:setting:rules:learned}
    (represented by recursive Datalog program).
\textcolor{gray}{ \st{Note that the analyzer accurately classifies most
    variables of the training corpus, and is also sound when applied
    to new programs.}
    }
}
  \label{fig:motivation:example}
  \vspace{-1em}
\end{figure*}


Consider the program in Fig.~\ref{sfig:motivation:example:program},
which computes the $\chi$ function from Keccak, a family of
cryptographic primitives for the SHA-3
standard~\cite{nist2012keccak,bertoni2012keccak}. It ultimately
computes the function 
%
\lstinline|n1 = i1 $\oplus$ ($\lnot$ i2 $\land$ i3)|,  
%
where $\oplus$ means XOR.
Unfortunately, a straightforward implementation could potentially leak
knowledge of the sensitive inputs \lstinline|i1|, \lstinline|i2| and
\lstinline|i3| if the attacker were able to guess the intermediate
results \lstinline|$\lnot$ i2| and \lstinline|$\lnot$ i2 $\land$ i3|
via the \emph{power}
side-channels~\cite{eldib2014synthesis,barthe2018maskverif}.  The
masking countermeasures in the implementation therefore use three
additional random bits \lstinline|r1|, \lstinline|r2| and
\lstinline|r3| to prevent exposure of the private inputs while still
computing the desired function.

\setlength{\textfloatsep}{10pt plus 1.0pt minus 2.0pt}
\begin{figure}[t]
 \centering
\footnotesize{
  %\begin{subfigure}[b]{0.48\textwidth}
  \subfloat[Excerpt of rules learned by the \GPS{} tool.]
  {
    %\begin{equation*}
    $
      \begin{array}{rrcl}
        R_1: & \RUD(x) & \gets & \XOROP(x) \land \RCOP(x, R) \land \RUD(R) \land \lnot f(x) \\
        R_2: & \textcolor{red}{f(x)} & \gets & \LCOP(x, L) \land \RCOP(x, R) \land g_1(L, r_L) \land \\
             &      &        & g_2(R, r_R) \land r_L = r_R \\
        R_3: & g_1(r, r) & \gets & \INRANDOP(r) \\
        R_4: & g_1(x, r) & \gets & \LCOP(x, y) \land g_1(y, r) \\
        R_5: & g_1(x, r) & \gets & \RCOP(x, y) \land g_1(y, r) \\
        R_6: & g_2(r, r) & \gets &\INRANDOP(r) \\
        R_7: & g_2(x, r) & \gets & \LCOP(x, y) \land g_2(y, r) \land \XOROP(x) \\
        R_8: & g_2(x, r) & \gets & \RCOP(x, y) \land g_2(y, r) \land \XOROP(x) 
      \end{array}
    $ 
    %\end{equation*}
    \label{sfig:motivation:setting:rules:learned}
  }
  \vspace{1ex}
    
  %\begin{subfigure}[b]{0.48\textwidth}
  \subfloat[Corresponding expert written rules from SCInfer~\cite{zhang2018sc}.]
  {
    %\begin{equation*}
    $
      \begin{array}{rrcl}
        M_1: & \RUD(x) & \gets & \XOROP(x) \land \DOMOP(x, \text{res}) \land \text{res} \neq \emptyset \\
        M_2: & \SUPPOP(x, x) & \gets & \INRANDOP(x) \lor \INKEYOP(x) \lor \INPUBOP(x) \\
        M_3: & \SUPPOP(x, \text{res}) & \gets & \LCOP(x, L) \land \RCOP(x, R) \land \SUPPOP(L, S_L) \land \\
             &  &  & \SUPPOP(R, S_R) \land \text{res} = S_L \union S_R \\
        M_4: & \DOMOP(x, x) & \gets & \INRANDOP(x) \\
        M_5: & \DOMOP(x, \emptyset) & \gets & \INKEYOP(x) \lor \INPUBOP(x) \\
        M_6: & \DOMOP(x, \text{res}) & \gets & \XOROP(x) \land \LCOP(x, L) \land \RCOP(x, R) \land \\
             &    &    & \DOMOP(L, S_{DL}) \land \DOMOP(R, S_{DR}) \land \\
             &    &    & \SUPPOP(L, S_L) \land \SUPPOP(R, S_R) \land \\
             &    &    & \text{res} = (S_{DL} \union S_{DR}) \setminus (S_L \union S_R)
      \end{array}
    $
    %\end{equation*}
    \label{sfig:motivation:setting:rules:scinfer}
  }
}
  % TODO: State the meaning of f(x) and g(x, y) in English.
  \caption{Comparing the rules learned by \GPS{}
    (Fig.~\ref{sfig:motivation:setting:rules:learned}) to manually
    crafted rules from SCInfer
    (Fig.~\ref{sfig:motivation:setting:rules:scinfer}). 
    \textcolor{gray}{
    \st{$\LCOP(x, L)$ and $\RCOP(x, R)$ 
    indicate that the AST nodes $L$ and $R$ are
    the left and right operands of $x$ respectively.}
    \st{By default, every variable is of distribution type $\UKD$ unless specifically elevated to $\SID$ or $\RUD$ by a learned rule.  }
    }
    Observe that the learned rules are \emph{sound}, i.e., every variable which potentially leaks information is assigned the distribution type $\UKD$, while still managing to draw non-trivial conclusions such as $\RUD(\mathlst{b4})$.
    \textcolor{red}{The learned rules ($R_2$---$R_8$) in Fig.~\ref{sfig:motivation:setting:rules:learned} are used
     to define the new feature $f(x)$ in Fig.~\ref{sfig:motivation:example:tree4}}.
    %Furthermore, the learned rules (Fig.~\ref{sfig:motivation:setting:rules:learned}) have complex structure, including unspecified intermediate predicates such as $f(x)$ and $g(x, y)$, but are still orders of magnitude faster than the corresponding rules from the expert-written analysis.
    }
  \label{fig:motivation:setting:rules}
\end{figure}

\begin{figure*}
\centering
\subfloat[]
{
  \begin{minipage}[c][1\width]{0.32\textwidth}
	   \centering
           \input{images/motivation/features.tex}
           \vspace{-1.5ex}
	\end{minipage}
  \label{sfig:motivation:synthesis:features:predefined}
}
\hfill
\hspace{-1.25em}
\subfloat[] 
{
  \begin{minipage}[c][1\width]{0.32\textwidth}
    \centering
    \scalebox{0.7}{\input{images/motivation/tree1.tex}}
    \vspace{-1.5ex}
  \end{minipage} 
  \label{sfig:motivation:synthesis:features:tree1}
}
\hfill
\hspace{-1.75em}
\subfloat[] 
{
  \begin{minipage}[c][1\width]{0.32\textwidth}
	   \centering
	   \scalebox{0.7}{\input{images/motivation/tree2.tex}}
	   \vspace{-1.5ex}
	\end{minipage}
  \label{sfig:motivation:synthesis:features:tree2}
}
\caption{
  %Pre-defined features available to the rule learning algorithm,
  %categories into which it classifies intermediate program results
  %(Figure~\ref{sfig:motivation:synthesis:features:predefined}), and
  %the classifier learned only using these features
  %(Figure~\ref{sfig:motivation:synthesis:features:tree1}).  In
\textcolor{gray}{
  \st{The white nodes of Fig
  represent pre-defined features, while the grey nodes represent output classes
  (associated types).}
}
%
  The classifier of
  Fig.~\ref{sfig:motivation:synthesis:features:tree1} is learned
  only using the features in
  Fig.~\ref{sfig:motivation:synthesis:features:predefined}.  Because
  of the limited expressive power of these features, the learned
  analysis necessarily misclassifies either \lstinline|b4| or
  \lstinline|n1|. 
%
  Fig.~\ref{sfig:motivation:synthesis:features:tree2}
  denotes the candidate analyzer produced after one round of
  feature synthesis. The blue paths corresponds to the rule $\RUD(x) 
  \gets \XOROP(x) \land \XOROP(R) \land \RUD(L) \land \lnot f(x) 
  \land LC(x, L) \land RC(x, R)$. Unfortunately, even though 
  this analysis (Fig.~\ref{sfig:motivation:synthesis:features:tree2}) achieves 100\%
  training accuracy, the leaf nodes highlighted in red correspond to
  unsound predictions.  
  }
\label{fig:motivation:synthesis:features}
\vspace{-1em}
\end{figure*}

\input{motivation-setting.tex}
\input{motivation-synthesis.tex}
\input{motivation-proof.tex}

%\input{motivation-architecture.tex}


==> overall.tex <==
\section{The Overall Algorithm}
\label{sec:overall}

In this section, we present the overall algorithm
(Algorithm~\ref{alg:overall}), which takes the example set
$\mathcal{E}$ and the feature set $\mathcal{F}$ as input and returns
the learned analyzer as output.
%
First, the learner is invoked to learn a set $R$ of inference rules.
Then, the set $R$ is given to the prover for verification.
%
Proved rules will be added to the analyzer, whereas rules that cannot
be proved will be dropped.
%
If no rule in $R$ gets rejected, it returns the analyzer $A_i$.
%
Let $R_{rej}$ be the set of dropped rules.  For each rule $\alpha\in
R_{rej}$, we construct a counterexample $\mathcal{E}_\alpha$, and add
it back to the example set $\mathcal{E}$.



\begin{algorithm}[t]
\input{images/overall/overall.tex}
\caption{The Overall Algorithm.}
\label{alg:overall}
\end{algorithm}





Consider a dropped rule $R_{rej}$ as follows:
$\mathbb{SID}(x) \leftarrow \mathbb{XOR}(x)$ $\wedge~\mathbb{XOR}(L) \wedge
\mathbb{XOR}(R) \wedge \mathbb{RUD}(L) \wedge \mathbb{RUD}(R)$. 
%
Since we want to generate a counterexample to prevent the $learner$
from learning the same $R_{rej}$ again, we add the last row (in
red-colored text) to the Table in Figure~\ref{fig:learner:feature-val}.
%
The new row has the same feature values as in the body of $R_{rej}$,
together with a different head value; that is, the head value is
changed conservatively from $\mathbb{SID}$ to $\mathbb{UKD}$.
%
%
For features that are not used in the body of $R_{rej}$, we would set
their values to -1 (meaning \emph{not applicable}). 


Inside DTL, when we compute the conditional entropy of a feature whose
corresponding value is -1 (not applicable), we simply skip this
example (e.g., a row of the Table in Figure~\ref{fig:learner:feature-val}).  
%
In other words, the counterexample derived from $R_{rej}$ is an
abstract example, as opposed to a concrete example from the training
data set.  Nevertheless, it provides a succinct and efficient way to
prevent the learner from generating $R_{rej}$ again. 

%%%%%%%%%%%%
\begin{comment}
\begin{table}
\caption{Illustration of Negative Example Generation.}
\vspace{-1em}
\footnotesize
\begin{tabular} {|c|c|c|c|c|c|c|}
\hline
$\mathcal{E}$ & $F_1$ & $F_2$ & $F_3$ & $F_4$ & $F...$ & $\mathbb{TYPE}$
\\ \hline \hline
$\mathcal{E}_1$ &1 & 1 & 0 & 1 & 1 & $\mathbb{RUD}$
\\ \hline
$\mathcal{E}_2$ & 1 & 0 & 0 & 1 & 0 & $\mathbb{RUD}$
\\ \hline
$\mathcal{E}_3$ &  0 & 0 & 0 & 1 & 1 & $\mathbb{UKD}$
\\ \hline
$\mathcal{E}_{\alpha}$ & \textcolor{red}{1} & \textcolor{red}{1} & \textcolor{red}{0} & \textcolor{red}{1} & \textcolor{red}{-1} & $\textcolor{red}{\mathbb{UKD}}$
\\ \hline
\end{tabular}
\vspace{-2em}
\label{CounterExample}
\end{table}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%


==> prelims.tex <==
\section{Preliminaries}
\label{sec:prelims}

%We review the basics of \emph{power} side channels and type
%systems.


\subsection{Power Side-Channels}

Prior works~\cite{ishai2003private,balasch2014cost,coron2012conversion}
%
show that variance in the power consumption of a computing device may
leak secret information; for example, when a secret value is stored in
a physical register, its number of logical-1 bits may affect the power
consumption of the CPU.  Such side-channel vulnerabilities are
typically mitigated by \emph{masking}, e.g., using random bits
($r_1,\ldots,r_{d}$) to split a secret $key$ bit into $d + 1$ shares:
$key_1 = r_1$, $key_2 = r_2$, $\ldots$, $key_{d+1} = r_1 \oplus r_2
\ldots \oplus r_d \oplus key$, where $\oplus$ denotes the logical operation \emph{exclusive or} (XOR).  Since all
$d+1$ shares are uniformly distributed in the $\{0,1\}$, in theory, this
\emph{order-d masking} scheme is provably secure in that any combination of
less than $d$ shares cannot reveal the secret, but combining all $d+1$
shares, $key_1 \oplus key_2 \oplus ... key_{d+1}$ = $key$, recovers
the secret.


In practice, masking countermeasures must also be implemented properly to avoid
de-randomizing any of the secret shares accidentally.  Consider $t$ =
$t_L \oplus t_R$ = ($r_1 \oplus key$) $\oplus$ ($r_1 \oplus b$) = $key
\oplus b$.  While syntactically dependent on the two randomized values
$t_L$ and $t_R$, $t$ is in fact leaky because, semantically, it does
not depend on the random input $r_1$.
%
In this work, we aim to learn a static analyzer that can soundly prove
that \emph{all intermediate program variables} are free of such
leaks.



\subsection{Type Systems}
\label{typeSys}


Type systems prove to be effective in analyzing power side
channels~\cite{zhang2018sc,wang2019mitigating}, e.g., by certifying
that all intermediate variables of a program are \emph{statistically
  independent} of the secret.
%
Typically, the program inputs are marked as public (\texttt{INPUB}),
secret (\texttt{INKEY}) or random (\texttt{INRAND}), and then the
types of all other program variables are inferred automatically. 


The type of a variable $v$, denoted \texttt{TYPE(v)}, may be
\texttt{RUD}, \texttt{SID}, or \texttt{UKD}.
%
Here, \texttt{RUD} stands for random uniform distribution, meaning $v$ is either a random bit or being masked by a random bit.
%
\texttt{SID} stands for secret independent distribution, meaning 
$v$ does not depend on the secret.
%
\texttt{UKD} stands for unknown distribution, or potentially leaky; if
the analyzer cannot prove $v$ to be \texttt{RUD} or \texttt{SID}, then
it is \texttt{UKD}.



Type systems are sound but not necessarily complete.  
%
They are sound in that they never miss real leaks. 
%
For example, by default, they may safely assume that all variables are
\texttt{UKD}, unless a variable is specifically elevated to $\SID$ or $\RUD$ 
by an analysis rule.
%unless a variable can be proved to be otherwise.
%
Similarly, they may conservatively classify \texttt{SID} variables as
\texttt{UKD}, or classify \texttt{RUD} variables as \texttt{SID},
without missing real leaks. 
%
In general, the sets of variables marked as the three types form a
hierarchy: $S_{\texttt{RUD}}$ $\subseteq$ $S_{\texttt{SID}}$
$\subseteq$ $S_{\texttt{UKD}}$.

\textcolor{red}{
\subsection{Relations}
}
\textcolor{red}{
The program (in SSA format) is represented 
as the abstract syntax tree (AST).
Static analyzers infer the type of 
each node $x$ of the program's AST
based on various \emph{features} of $x$.
In this work, pre-defined features are represented as
\emph{relations}.
%
\begin{itemize}
\item 
Unary relations $\INPUBOP(x)$, $\INKEYOP(x)$, and $\INRANDOP(x)$
denote the given security level of a program input $x$, which may be
public, secret, or random.
\item 
Unary relations $\RUD(x)$, $\SID(x)$, and $\INRANDOP(x)$ denote the
inferred type of a program variable $x$, which may be uniformly
random, secret independent, or unknown.
\item 
Unary relation $\OPOP(x)$ denotes the operator type of the AST node
$x$, e.g., $\OPOP(x)$ := $\ANDOROP(x)$~$|$~$\XOROP(x)$, where
$\ANDOROP(x)$ means that $x$'s operator type is either \emph{logical
  and} or \emph{logical or}, and $\XOROP(x)$ means that $x$'s operator
type is \emph{exclusive or};
\item 
Binary relations $\LCOP(x,L)$ and $\RCOP(x, R)$ indicate that the AST
nodes $L$ and $R$ are the left and right operands of $x$,
respectively.
%
\item 
Binary relation $\SUPPOP(x,y)$ indicates that the AST node $y$ is used
in the computation of $x$ syntactically, while $\DOMOP(x,y)$ indicates
that random variable $y$ is used in the computation of $x$
semantically.
\end{itemize} 
}
%
%



==> prover-alpha.tex <==
\subsection{Representation of the Learned Rule ($\alpha$)}
\begin{figure}
\centering
\scalebox{0.85}{\input{images/prover/AST_proof.tex}}
\vspace{-.5em}
\caption{Example $AST$ from which $\alpha$ is learned.}
\label{proofAST}
%\vspace{-1em}
\end{figure}

Let $\alpha$ be a set of Datalog rules, each of which has a head
relation $\phi_{\alpha}$ and a body of the following form:
%
%\begin{center}
%$ P_0(x,y) \leftarrow  P_1(x,x_1) \wedge P_2(x_1,x_2), \ldots, \wedge P_k(x_{k-1},y)$
%\end{center}
%
\begin{alignat}{1}
  \phi_{\alpha}(\bm{x}) & \gets \phi_1(\bm{x}_1) \land \phi_2(\bm{x}_2) \land \dots \land
                                   \phi_n(\bm{x}_n)
\end{alignat}
It means $\phi_{\alpha}$ holds only when all of $\phi_1,\ldots,\phi_k$ hold.
%Furthermore, 
%while $P_1,\ldots,P_k$ may be both intensional (learned)
%and extensional (predefined) attributes, 
%$P_0$ can only be an learned attribute.
%intensional (learned) attribute.  
%
Here, $\phi_{\alpha}$ may be a distribution type, e.g., $\SID(x)$, or
a recursive feature $g(x,y)$, e.g.,  representing that $x$ depends on $y$.
%
%Although the algorithm~\ref{alg:learner} guarantees that all learned rules are
%mostly consistent with the training programs, the rules are not always generalizable
% to other programs.
%
%For instance, it is possible for a new program, whose root
%is not $\SID(x)$, to satisfy a rule for $\SID(x)$.
%%
%In such a case, we must drop the rule.


==> prover-cex.tex <==
\subsection{Generating Abstract Counter-Examples}
\label{sub:prover:cex}

When the proof fails, however, we need to prevent the same rule from
being learned again. 
%
%Recall that the analysis learned by $\DTL(\mathcal{E}, \mathcal{F})$
%is a decision tree whose leaves classify the AST nodes as $\RUD(x)$,
%$\SID(x)$, or $\UKD(x)$. Each path to a leaf node corresponds to a
%Datalog program which will be subject to verification by the algorithm
%descibed in the previous section. The \GPS{} tool successfully
%terminates when this check succeeds.
%
%
%
Let $\pi = \{ f_1 = v_1, f_2 = v_2, \dots, f_k = v_k \}$ be the feature valuation in the failing
rule $R_\pi$. We then construct the counter-example,
\begin{alignat}{1}
  CE_\pi & = \{ f \mapsto v \mid (f, v) \in \pi \} \union \{ f \mapsto -1 \mid f \in \mathcal{F} \setminus \pi \}
\end{alignat}
with label $\UKD(CE_\pi)$. Recall that $\mathcal{F}$ is the set of all features currently under consideration. 
%Notice
%that since the verifier is a semi-decision procedure, we are unable to construct a concrete counter-example for which
%the candidate analysis $\alpha$ produces unsound results. 
Therefore, the feedback $CE_\pi$ provided to
$\DTL(\mathcal{E}, \mathcal{F})$ is an \emph{abstract} counter-example, with the missing features $f \in \mathcal{F} \setminus
\pi$ set to the unknown value $-1$.

Consider the subsequent iteration of the decision tree learner, $\DTL(\mathcal{E} \union \{ CE_\pi \}, \mathcal{F})$.
Observe that whenever it is in a decision context which is also a prefix $\pi_{pre}$ of the  counter-example
$CE_\pi$, the information gain of each feature $f \in \pi$ is strictly less than that encountered in the previous
invocation. Therefore, at some level of the decision tree, it will either choose a different feature, or invoke the feature synthesis algorithm to grow $\mathcal{F}$. By formalizing this argument, we say that:
\begin{proposition}
Given a counter-example $CE_\pi$ to a learned rule $R_\pi$, the subsequent invocation of the learner $\DTL(\mathcal{E} \union \{ CE_\pi \}, \mathcal{F})$ is guaranteed to no longer produce $R_\pi$.
\end{proposition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 1. Iterative procedure, why we need counter-examples
% We could also restore soundness by silently dropping rules for which the soundness check fails

% The \emph{prover} unveils the unsound rules by the containment checking, and yields the remaining sound rules. However,
% the \GPS{} tool would not terminate via merely outputting the provably sound rules after one-shot learning. As shown in
% Figure~\ref{sfig:motivation:synthesis:features:tree2}, the learned decision tree after first iteration consists of two
% sound rules while the remaining five rules are verified as unsound. These two rules are insufficient to correctly
% classify a large corpus of the variables despite being provably sound, and thereby notoriously harms the accuracy of the
% analysis. To improve the accuracy while guaranteeing soundness, we propose an abstract way to generate the
% counterexamples, prohibiting \emph{learner} from generating the same rejected rules in next iteration. Along with the
% \emph{prover} and counterexample generation, we scale the decision tree learning from one-shot to multiple shots. This
% gradually refined learning process is analogous to the regularization in machine learning area, where we impose more
% examples to enhance generalization and avoid overfitting. Here, the soundness constraint is like a regularization term
% imposed in the objective function.


==> prover-ind.tex <==
\subsection{Proving the Soundness of $\alpha$ Using $KB$}
\label{sub:prover:ind}

To prove that for every AST node $x$ marked as $\RUD_\alpha(x)$
(resp. $\SID_\alpha(x)$) by $\alpha$, it is also marked as
$\RUD_{KB}(x)$ (resp. $\RUD_{KB}(x)$) by $KB$, we show that the
following relation $Ind(x)$ is empty for any valuation of the input
relations:
\begin{alignat}{1}
  Ind(x) & \gets \phi_\alpha(x) \land \lnot \phi_{KB}(x) ~,
\end{alignat}
where the relation $\phi$ may be instantiated to either $\RUD$ or
$\SID$.
%
%
In theory, this amounts to proving \emph{query containment}, which is
undecidable for Datalog in general~\cite{calvanese2005decidable,
  calvanese1998decidability}, but there are Datalog fragments, such as
UC2RPQ, for which it is decidable~\cite{calvanese2005decidable,
  calvanese2003reasoning, barcelo2014does} and our meta-rules in
Fig.~\ref{fig:learner:sygus:metarules} were designed specifically to
produce rules within this fragment.



\ignore{%% chao: I wonder if we can move the following paragraphs to the appendix

In the remainder of this section, we present a semi-decision procedure
to prove the emptiness of $Ind(x)$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 1. Derivation Trees and Inlining Depths

\paragraph{Derivation trees, and unrolling a Datalog program}

First, we observe that every tuple $t = \phi(x)$ produced by a Datalog program is associated with one or more
\emph{derivation trees}. %such as that shown in Figure~\ref{}. 
The heights of these derivation trees correspond to the
depth of rule inlining at which the program discovers $t$. In particular, for each inlining depth $k \in \N$, each rule
$\phi_h(\bm{x}_h) \gets \phi_1(\bm{x}_1) \land \phi_2(\bm{x}_2) \land \dots \land \phi_n(\bm{x}_n)$ can be transformed to
\begin{alignat}{1}
  \phi^{(k + 1)}(\bm{x}_h) & \gets \phi^{(k)}_1(\bm{x}_1) \land \phi^{(k)}_2(\bm{x}_2) \land \dots \land
                                   \phi^{(k)}_n(\bm{x}_n), \label{eq:prover:ind:unrolling}
\end{alignat}
where each $\phi^{(k)}$ contains exactly those tuples $\phi^{(k)}(\bm{x})$ which have a derivation
tree of depth $k$. Observe that $\phi = \bigcup_{k \in \N} \phi^{(k)}$.

% TODO: Figure of derivation tree

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 2. Strengthening the Goal, and the Fundamental Proposition

\paragraph{Proving entailment at each unrolling depth.}

Our insight is to prove that at each unrolling depth $k$, $\phi^{(k)}_\alpha \subseteq \phi^{(k)}_{KB}$. In other words,
we define the relation $Ind^{(k)}$ as follows:
\begin{alignat}{1}
  Ind^{(k)}(x) \gets \phi^{(k)}_\alpha(x) \land \lnot \phi^{(k)}_{KB}(x), \label{eq:prover:ind:approx}
\end{alignat}
and extrapolate from the emptiness of $Ind^{(k)}$ for each $k$:
\begin{proposition}
If $Ind^{(k)}(x)$ is an empty relation for each inlining depth $k \in \N$, then $Ind(x)$ is also an empty relation.
\end{proposition}
\begin{proof}
Assume otherwise, so the $Ind$ relation contains some AST node $x$. By definition then, the candidate analysis $\alpha$
derives $\phi_\alpha(x)$, say at proof tree depth $l$, while $KB$ does not derive $\phi_{KB}(x)$. It follows that
$\phi^{(l)}_\alpha$ also contains $x$, and that $\phi^{(l)}_{KB}$ is an empty relation. We conclude that $x$ is an
element of $Ind^{(l)}$, which contradicts our hypothesis that $Ind^{(l)}$ was empty.
\end{proof}

\begin{note}
The converse of the above proposition need not hold. In particular, it may be the case that $Ind(x)$ is empty, even
though $Ind^{(k)}$ is inhabited. This is a curious consequence of connecting the inlining depths of $\phi_\alpha$ and
$\phi_{KB}$ in Equation~\ref{eq:prover:ind:approx}: there may be a tuple $\phi^{(k)}_\alpha(x)$ which is derived by $KB$
at some other inlining depth $k' \neq k$. In that case, since $x$ would then be absent from $\phi^{(k)}_{KB}(x)$, it
would inhabit $Ind^{(k)}(x)$, but not occur in $Ind(x)$.
\end{note}

}%\ignore{}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 3. k-induction.
% Note that k-induction can be done by a sequence of queries to an SMT solver
% For k = 1 to infinity, do ...

%\paragraph{Mechanizing the soundness proof by $k$-induction}

Specifically, we prove the emptiness of $Ind(x)$ by $k$-induction~\cite{sheeran2000checking,
  donaldson2011software, gadelha2017handling}.
%
Observe that unrolling the rules of a Datalog program to any specific depth yields a formula which can be interpreted
within propositional logic. For example, unrolling $f(x)$ from Equation~\ref{eq:learner:sygus:zeroGain} at depths $1$
and $2$ gives us
{%\footnotesize
\begin{alignat*}{1}
  f^{(1)}(x) & = \INRANDOP(x), \text{ and} \\
  f^{(2)}(y) & = (\LCOP(y, x) \land f^{1}(x)) \lor (\RCOP(y, x) \land f^{1}(x)).
\end{alignat*}
}%
%
For any specific value of $k$, we can therefore use an SMT solver to verify the emptiness of 
$Ind^{(k)}$ for all $k=1,2,\ldots$.

For the inductive step, in particular, we ask the SMT solver to
determine if $Ind^{(i + k)}$ can be non-empty while the $k$ preceding
relations $Ind^{(i)}$, $Ind^{(i + 1)}$, $Ind^{(i + 2)}$, \dots,
$Ind^{(i + k - 1)}$ are all empty. For this purpose, let $V^{(i)}$ be
free variables introduced by unrolling the rules at depth $i$. The
following formula asserts the non-emptiness of $Ind^{(i)}$:
\begin{alignat}{1}
  \Phi^{(i)} & = \bigvee_{x \in V^{(i)}} Ind^{(i)}(x).
\end{alignat}
Thus, we formalize the inductive step of the proof by constructing the following formula:
\begin{alignat}{1}
  \Psi^{(k)} & = \lnot \Phi^{(i)} \land \lnot \Phi^{(i + 1)} \land \dots \land \lnot \Phi^{(i + k - 1)} \land \Phi^{(i + k)}
\end{alignat}
%
%
The following proposition formalizes our intuition:
\begin{proposition}
\label{prop:prover:ind:k}
If for some $k \in \N$, the relations $Ind^{(1)}$, $Ind^{(2)}$, \dots, $Ind^{(k)}$ are all empty, and the formula
$\Psi^{(k)}$ is unsatisfiable, then $Ind^{(i)}$ is empty for all $i \in \N$.
\end{proposition}
Starting from $k = 1$, we use the SMT solver to check Proposition~\ref{prop:prover:ind:k} for increasingly larger $k$ until a timeout is reached. If the SMT solver is ever successful in proving the proposition, it follows that
the learned rule $\alpha$ is sound.


==> prover-kb.tex <==
\input{kb_distribution}

\subsection{Representation of the Knowledge Base ($KB$)}
\label{sub:prover:kb}

Our $KB$ consists of two sets of proof rules, one for propositional
logic and the other for distribution types. 

\emph{Proof Rules for Propositional Logic}
Fig.~\ref{boolean} shows the proof rules that represent axioms of
propositional logic~\cite{russell2002artificial}; they can be used to reduce any valid
(resp. invalid) Boolean formula to constant $true$ (resp. $false$).
%
Thus, they are useful in showing results such as $true \vee P$ and
$false \wedge Q$ are secret-independent ($\SID$), for arbitrary
logical sentences $P$ and $Q$.


Consider the example rule $\alpha$ below, where $g_1$ and $g_2$ are
synthesized features shown as dashed boxes in Fig.~\ref{proofAST}:
\begin{tabular}{@{\hskip3pt}c@{\hskip3pt} c @{\hskip3pt}l@{\hskip3pt}}
{\footnotesize $\SID$($x$)} & {\footnotesize$\leftarrow$} & {\footnotesize $\OROP$($x$) $\wedge$ $\LCOP$($x$, $L$) 
$\wedge$ $\RCOP$($x$, $R$) $\wedge$ $\OROP$($L$)
$\wedge$ $\NOTOP$($R$) $\wedge$ } \\
 & & {\footnotesize $g_1$($L$, $k_1$)
$\wedge$ $g_2$($R$, $k_2$) $\wedge$ $\texttt{EQ}(k_1,k_2)$} \\
{\footnotesize $g_1$($L$, $k_1$)}& {\footnotesize $\leftarrow$} & 
{\footnotesize $\INKEYOP$($k_1$) $\wedge$ $\INRANDOP$($r_1$) $\wedge$ $\LCOP$($L$, $k_1$) $\wedge$ $\RCOP$($L$, $r_1$)} \\
{\footnotesize $g_2$($R$, $k_2$)} & {\footnotesize $\leftarrow$} & 
{\footnotesize $\INKEYOP$($k_2$) $\wedge$ $\LCOP$($R$, $k_2$) }
\end{tabular}

\noindent
%
Since $k_1=k_2$, we transform $\alpha$ into an equivalent logic formula: 
\begin{center}
{\footnotesize
$\SID(x) \leftarrow \texttt{EQ}(x, (k_1 \vee r_1) \vee (\neg k_1)) $ 
}
\end{center}
%
Rules $B1$, $B7$ and $Bf$ in Fig.~\ref{boolean} show that
$(k_1 \vee r_1) \vee (\neg k_1)$ is always $true$.  Thus, $x$ is
always $true$.  Since $x$ is a constant, we have $\SID$($x$), meaning $x$
is secret-independent.
%\begin{center}
%\footnotesize{
%$x$ $\vee$ $y$ $\vee z$ = $x$ $\vee$ $z$ $\vee$ $y$, $x$ $\vee$ $\neg x \rightarrow$ $True$, 
%$x$ $\vee$ $True \rightarrow$ $True$
%}
%\end{center}

Such seemingly simple $\SID$ rules, learned by our method
automatically, and yet overlooked by state-of-the-art (hand-crafted)
analyzers~\cite{zhang2018sc,wang2019mitigating}, can significantly
improve the accuracy of side-channel analysis on many programs.  


\ignore{
%
Note that repeated application of the rules shown in
Figure~\ref{boolean} is not guaranteed to terminate.  The analysis
basically infers more equality relations by repeatedly applying the
equality analysis rules in Figure~\ref{boolean}, with the help of
saturation engine~\cite{tate2009equality,kovacs2013first}.
Non-termination may happen when the equality saturation engine never
gets out of the equality analysis.  The axioms $B_6$: $b \vee false
\equiv b$ used in the direction from right to left can be applied
infinite times, generating successively larger expressions $(b, b \vee
false, (b \vee false) \vee false, ...)$.  As opposed to using
Figure~\ref{boolean} as analyzer, here we leverage the rules of
Figure~\ref{boolean} as the \emph{prover}, we are trying to prove the
following rule:
%
\begin{alignat}{1}
  \SID_{\alpha}(\bm{x}) & \gets \phi_1(\bm{x}_1) \land \phi_2(\bm{x}_2) \land \dots \land
                                   \phi_n(\bm{x}_n)
\end{alignat}
In the above rule, assuming that $\mathcal{S}$ represents the set of clauses in the body and more clauses
get added to $\mathcal{S}$ after applying equality analysis rules. 
%
As long as that there exists one constant clause ($true,
false$) transformed from the body of the original rule, the \emph{prover}
can terminate and validate the soundness. Otherwise, it would transfer
the soundness checking to the more comprehensive distribution rules
after hitting the timing bound.
}

%These are based on proof rules gathered from prior
%works~\cite{zhang2018sc,eldib2014synthesis,barthe2015verified},
%previously used to prove that masking countermeasures have no leaks.
%We enhanced them by adding similar rules to handle more special cases.
%
\ignore{
%% Chao: ignored the following paragraph, since it gives the 
%impression that rules in $KB$ are also used in the analyzer, and 
%thus $KB$ itselfs can act as an analyzer
%
While it is straightforward to add new rules to $KB$, in general, it
is difficult to know how useful each rule is in the analyzer.  
%
While adding too many inference rules to the analyzer is risky, e.g.,
it may drastically slow down the analyzer without bringing noticeable
increase in accuracy, adding them to $KB$ does not have such risk,
since $KB$ is used to prove the validity of $\alpha$ only during the
learning phase.
}%\ignore{}
%
\emph{Proof Rules for Distribution Types.}  Fig.~\ref{fig:kbRule}
shows the proof rules that represent properties of the distribution
types.  They were collected from published
papers~\cite{zhang2018sc,eldib2014synthesis,barthe2015verified} that
focus on verifying masking countermeasures, which also provided the
soundness proofs of these rules.  For brevity, we omit the detailed
explanation. Instead, we use Rule~$D_{2.3}$ as an example to
illustrate the rationale behind these proof rules.



In Rule $D_{2.3}$, the $dom$($x$, $S$) relation means $x$ is masked by
some input from the set $S$ of random inputs.
%
For example, in $y = x_1 \oplus x_2$, where $x_1 = k \oplus r_1 \oplus
r_2$ and $x_2 = b \oplus r_2$, we say that $x_2$ is masked by $r_2$,
and $x_1$ is masked by both $r_1$ and $r_2$.
%
However, since $r_2\oplus r_2 = false$, $y$ is masked only by $r_1$.
Thus, $dom$($y$, \{$r_1$\}) holds, but 
$dom(y,\{r_2\})$ does not hold.


In this sense, Rule $D_{2.3}$ defines a \emph{masking set}. For $y$, it is $S_y$ = (\{$r_1$, $r_2$\} $\cup$ \{$r_2$\}) $\setminus$ (\{$r_1$,
$r_2$\} $\cap$ \{$r_2$\}) = \{$r_1$\}, which contains $r_1$ only.
%
%
The masking set defined by $D_{2.3}$ is useful in that, as long as the
set is not empty, the corresponding variable is guaranteed to be
of the $\RUD$ type.



\ignore{
Even though these distribution rules are tailored to correctly
and soundly deriving the comprehensive examples cases as
compared with rules in Figure~\ref{boolean}, it still
remains constrained in deriving the constant case, such as the AST example
shown in Figure~\ref{proofAST} where the root variable $x$
is inferred as $\UKD$ by merely applying Figure~\ref{fig:kbRule},
since it's inapplicable to any distribution rule.
Therefore, our $KB$ encompasses propositional rules as well
as distribution rules, capable of verifying more $\SID$ rules
and $\RUD$ rules while maintaining soundness.
}


==> prover.tex <==
\section{Proving the Type-inference Rules}
\label{sec:prover}

%As we saw in Example~\ref{sfig:motivation:synthesis:features:tree2},
%even if the candidate analysis $\alpha$ learned by $\DTL(\mathcal{E},
%\mathcal{F})$ is consistent with all training examples, it may reach
%unsound conclusions when applied to new unseen programs.

We wish to prove that a learned rule, denoted $\alpha$, never reaches
unsound conclusions when applied to any program, by showing that it
can be deduced from a \emph{known-to-be-correct} knowledge base
($KB$).  More specifically, we wish to confirm that every AST node $x$
marked as $\RUD$ (or $\SID$) by $\alpha$ can be certified to be $\RUD$
(or $\SID$) by $KB$.
%
When both $\alpha$ and $KB$ are expressed in Datalog, the problem reduces
to one of determining query containment, e.g., for every valuation of
the input relations, $\RUD_\alpha \subseteq \RUD_{KB}$ (or $\SID_\alpha \subseteq \SID_{KB}$).
We will now describe a semi-decision procedure to verify the soundness of the learned rules $\alpha$, which forms the second phase of the synthesis loop in  \GPS{}.

\input{prover-alpha.tex} % \clearpage
\input{prover-kb.tex} % \clearpage
\input{prover-ind.tex} % \clearpage
\input{prover-cex.tex}


We stress that the \emph{proof rules} in $KB$ should not be confused with
\emph{analysis rules} used in the learned analyzer, since they are way more
computationally expensive.
%
Consider Rule~$D_{1.4}$, whose Datalog encoding size for $supp(x,S)$
would be $|V| \times 2^{|IN|}$.  For the benchmark named B19 in
Table~\ref{tbl:stats}, it owns 1250 input variables and thereby
causing the exponential explosion with $2^{1250}$.
%
The learned rule $\alpha$, in contrast, does not rely on these
expensive set (union and intersection) operations.


==> related.tex <==

\section{Related Work}
\label{sec:related}

\noindent
\textit{Generate Analyzers from Examples.}
%\paragraph{Generate Analyzers from Examples}
While there are prior works on learning static
analyzers~\cite{bielik2017learning,zaheer2016learning}, they do not
guarantee soundness.  For example, the analyzer learned by Bielik et
al.~\cite{bielik2017learning} is only sound with respect to the
programs in the training set, not all programs written in the same
programming language (JavaScript).  They also need to manually modify
the training programs to generate counter-examples, while our method
generates counter-examples automatically.

\noindent
\textit{Formal Specifications.}
%\paragraph{Formal Specifications} 
There are also works on synthesizing static analyzers from formal
specifications, e.g., proof rules or
second-order logic
formulas~\cite{david2015using,grebenshchikov2012synthesizing,
  chen2019vfql} as opposed to training data.
%
However, they restrict the logic used to write the formal
specification, and as a result, are not expressive enough to
synthesize practical analyzers. The users are also expected to
write correct specifications, which is a non-trivial task.  In
addition, they cannot exploit the information provided by
data.

\noindent
\textit{Learning-based Techniques.}
%\paragraph{Learning-Based Techniques} 
There are several prior techniques using machine learning to
conduct static program
analyses~\cite{katz2016estimating,raychev2015predicting,
  tripp2014aletheia,gvero2015synthesizing}.
%
Such techniques focus on finding a suitable program-to-feature
embedding. However, they require the user to perform feature
engineering, which is known to be laborious.
%
Some of these
techniques~\cite{mangal2015user,raychev2015predicting,heo2018adaptive,heo2016learning}
do not even take advantage of new features that may be learned from
data; instead, they build classifiers based solely on existing
features.
%
In contrast, our method not only learn new analysis rules from data,
but also use SyGuS to synthesize new features automatically.


\noindent
\textit{Optimizing an Analyzer.}
%\paragraph{Optimizing an Analyzer} 
%Instead of learning a new analyzer from data, there are techniques for
It is also possible to optimize an existing static
analyzer~\cite{grigore2016abstraction,
  heo2019resource,oh2015learning,heo2017machine,singh2018fast,katz2016estimating},
%
which can be achieved by adjusting the level of
abstraction~\cite{grigore2016abstraction, heo2019resource}, learn
heuristics and parameters~\cite{oh2015learning}, make
soundness-accuracy trade-offs~\cite{heo2017machine}, or select sound
transformers~\cite{singh2018fast}.
%
However, such techniques fundamentally differ from our method because
they assume the analyzer is already given, and their focus is on
optimizing its performance, whereas we focus on synthesizing a new
analyzer.

\noindent
\textit{Syntax-Guided Synthesis.}
%\paragraph{Syntax-Guided Synthesis} 
Since we automatically generate new features, our method is related to
the large and growing body of work on SyGuS.
%
While SyGuS has been used in various
applications~\cite{rolim2017learning,mechtaev2016angelix,feng2017component,
  polikarpova2016program,abate2017automated,
  bavishi2019phoenix,xiong2017precise,le2017s3,hua2018towards,
  knoth2019resource,li2015resource}, none of them aims to synthesize a
provably sound static analyzer from data.
%
While some of these existing techniques can synthesize Datalog
rules~\cite{si2018syntax,zhang2014abstraction,si2019synthesizing}, the
focus has been on efficiency, e.g., pruning the search space based on
syntactic structures, instead of guaranteeing the soundness of the
analyzer.


\noindent
\textit{Power Side-Channel Analysis.}
%\paragraph{Power Side-Channel} 
In this work, we use power side-channel analysis as the application to
evaluate our learning method.  In this sense, our work is related to
the body of work on detecting side-channel
leaks~\cite{chen2017precise,brennan2018symbolic,
  bang2016string,zhang2018sc} as well as mitigating
them~\cite{tizpaz2019quantitative,wang2019mitigating,
  cauligi2019fact,wu2018eliminating,eldib2014synthesis}.
%
While the static analysis engines used in these existing works are all
hand-crafted by domain experts, our method aims to synthesize the
static analysis from data automatically.

